Technical Design Report for the PANDA Barrel DIRC Detector

This documents describes the technical design and the expected performance of the Barrel DIRC detector for the PANDA experiment. The Barrel DIRC will provide hadronic charged particle identification in the polar angle range of $22^\circ$ to $140^\circ$ for particle momenta between 0.5 GeV/c and 3.5 GeV/c. The design is based on the successful BaBar DIRC with several key improvements. The performance and system cost were optimized in detailed detector simulations and validated with full system prototypes using particle beams at GSI and CERN. The final design meets or exceeds the PID goal of clean $\pi/K$ separation with at least 3 standard deviations over the entire phase space of charged kaons in the Barrel DIRC.

==> Makefile <==
DEFFILES=$(wildcard def_panda_*.tex)
TEXFILES=$(wildcard panda_tdr_*.tex)
#AUXFILES=$(patsubst %.tex, %.aux, $(TEXFILES)) 
AUXFILES=$(wildcard *.aux)
BBLFILES=$(patsubst %.aux, %.bbl, $(wildcard bu*.aux) )
BIBFILES=$(patsubst panda_tdr_dirc%.tex, lit_%.bib, $(TEXFILES) )
PNGFILES=$(wildcard *.pdf)

all:	test makeini panda_barrel_dirc.pdf


draft: $(BBLFILES)
	pdflatex "\def\classopts{,draft}\input{tdr-cherenkov}" -interaction=nonstopmode

test:
	@echo $(TEXFILES)
	@echo $(AUXFILES)
	@echo $(BIBFILES)
	@echo $(DEFFILES)
ifeq ($(strip $(BBLFILES)),) 
	@echo $(BBLFILES)
endif

pdf: panda_barrel_dirc.pdf

panda_barrel_dirc.pdf: $(BBLFILES) $(TEXFILES)
	pdflatex tdr-barrel-dirc.tex -interaction=nonstopmode


makeini: 
ifeq ($(strip $(BBLFILES)),) 
	@echo "initially TeXing..."
	pdflatex tdr-barrel-dirc.tex -draftmode -interaction=nonstopmode && make
endif


%.bbl:	%.aux
	- bibtex $<

#panda_tdr_hyper.aux: panda_tdr_hyper.tex
#	pdflatex panda_tdr_hyper.tex --shell-escape -draftmode

clean:
	- rm -f *.aux *.blg *.bbl *.log *.out *.toc *.lof

distclean: clean
	- rm -f panda_disc_dirc.pdf 

.PHONY: clean distclean test



==> collaboration/PANDA-LIST-July2015.tex <==
%
% PANDA Collaboration  - authorlist - automatically generated by PANDA website
2015-07-01 03:15:01\\[14pt] 
%
\institem{Aligarth Muslim University, Physics Department,{ \bf Aligarth}, India}
\authitem{B.~Singh}
\lastitem
\institem{Universität Basel,{ \bf Basel}, Switzerland}
\authitem{W.~Erni},
\authitem{I.~Keshelashvili},
\authitem{B.~Krusche},
\authitem{M.~Steinacher},
\authitem{N.~Walford}
\lastitem
\institem{Institute of High Energy Physics, Chinese Academy of Sciences,{ \bf Beijing}, China}
\authitem{B.~Liu},
\authitem{H.~Liu},
\authitem{Z.~Liu},
\authitem{X.~Shen},
\authitem{C.~Wang},
\authitem{J.~Zhao}
\lastitem
\institem{Universität Bochum, Institut für Experimentalphysik I,{ \bf Bochum}, Germany}
\authitem{M.~Albrecht},
\authitem{M.~Backwinkel},
\authitem{T.~Erlen},
\authitem{M.~Fink},
\authitem{F.~Heinsius},
\authitem{T.~Held},
\authitem{T.~Holtmann},
\authitem{S.~Jasper},
\authitem{I.~Keshk},
\authitem{H.~Koch},
\authitem{B.~Kopf},
\authitem{G.~Kuhl},
\authitem{M.~Kuhlmann},
\authitem{M.~Kümmel},
\authitem{S.~Leiber},
\authitem{M.~Leyhe},
\authitem{M.~Mikirtychyants},
\authitem{P.~Musiol},
\authitem{A.~Mustafa},
\authitem{M.~Pelizäus},
\authitem{J.~Pychy},
\authitem{M.~Richter},
\authitem{C.~Schnier},
\authitem{T.~Schröder},
\authitem{C.~Sowa},
\authitem{M.~Steinke},
\authitem{T.~Triffterer},
\authitem{U.~Wiedner}
\lastitem
\institem{Rheinische Friedrich-Wilhelms-Universität Bonn,{ \bf Bonn}, Germany}
\authitem{M.~Ball},
\authitem{R.~Beck},
\authitem{C.~Hammann},
\authitem{D.~Kaiser},
\authitem{B.~Ketzer},
\authitem{M.~Kube},
\authitem{P.~Mahlberg},
\authitem{M.~Rossbach},
\authitem{C.~Schmidt},
\authitem{R.~Schmitz},
\authitem{U.~Thoma},
\authitem{M.~Urban},
\authitem{D.~Walther},
\authitem{C.~Wendel},
\authitem{A.~Wilson},
\authitem{T.~Würschig}
\lastitem
\institem{Università di Brescia,{ \bf Brescia}, Italy}
\authitem{A.~Bianconi}
\lastitem
\institem{Institutul National de C\&D pentru Fizica si Inginerie Nucleara "Horia Hulubei",{ \bf Bukarest-Magurele}, Romania}
\authitem{M.~Bragadireanu},
\authitem{M.~Caprini},
\authitem{D.~Pantea},
\authitem{D.~Pietreanu},
\authitem{M.~Vasile}
\lastitem
\institem{P.D. Patel Institute of Applied Science, Department of Physical Sciences,{ \bf Changa}, India}
\authitem{B.~Patel}
\lastitem
\institem{IIT, Illinois Institute of Technology,{ \bf Chicago}, U.S.A.}
\authitem{D.~Kaplan}
\lastitem
\institem{University of Technology, Institute of Applied Informatics,{ \bf Cracow}, Poland}
\authitem{P.~Brandys},
\authitem{T.~Czyzewski},
\authitem{W.~Czyzycki},
\authitem{M.~Domagala},
\authitem{G.~Filo},
\authitem{T.~Gąciarz},
\authitem{M.~Hawryluk},
\authitem{J.~Jaworowski},
\authitem{M.~Krawczyk},
\authitem{D.~Kwiatkowski},
\authitem{F.~Lisowski},
\authitem{E.~Lisowski},
\authitem{M.~Michałek},
\authitem{P.~Poznański},
\authitem{J.~Płażek},
\authitem{Z.~Tabor}
\lastitem
\institem{IFJ, Institute of Nuclear Physics PAN,{ \bf Cracow}, Poland}
\authitem{B.~Czech},
\authitem{M.~Kistryn},
\authitem{S.~Kliczewski},
\authitem{K.~Korcyl},
\authitem{A.~Kozela},
\authitem{P.~Kulessa},
\authitem{P.~Lebiedowicz},
\authitem{K.~Pysz},
\authitem{W.~Schäfer},
\authitem{R.~Siudak},
\authitem{A.~Szczurek}
\lastitem
\institem{AGH, University of Science and Technology,{ \bf Cracow}, Poland}
\authitem{T.~Fiutowski},
\authitem{M.~Idzik},
\authitem{B.~Mindur},
\authitem{D.~Przyborowski},
\authitem{K.~Swientek}
\lastitem
\institem{Instytut Fizyki, Uniwersytet Jagiellonski,{ \bf Cracow}, Poland}
\authitem{J.~Biernat},
\authitem{S.~Jowzaee},
\authitem{B.~Kamys},
\authitem{S.~Kistryn},
\authitem{G.~Korcyl},
\authitem{W.~Krzemien},
\authitem{A.~Magiera},
\authitem{P.~Moskal},
\authitem{M.~Palka},
\authitem{A.~Pyszniak},
\authitem{Z.~Rudy},
\authitem{P.~Salabura},
\authitem{J.~Smyrski},
\authitem{P.~Strzempek},
\authitem{A.~Wronska}
\lastitem
\institem{FAIR, Facility for Antiproton and Ion Research in Europe,{ \bf Darmstadt}, Germany}
\authitem{I.~Augustin},
\authitem{I.~Lehmann},
\authitem{D.~Nicmorus Marinescu},
\authitem{L.~Schmitt},
\authitem{V.~Varentsov}
\lastitem
\institem{GSI Helmholtzzentrum für Schwerionenforschung GmbH,{ \bf Darmstadt}, Germany}
\authitem{M.~Al-Turany},
\authitem{R.~Arora},
\authitem{H.~Deppe},
\authitem{R.~Dzhygadlo},
\authitem{A.~Ehret},
\authitem{H.~Flemming},
\authitem{A.~Gerhardt},
\authitem{K.~Götzen},
\authitem{A.~Gromliuk},
\authitem{L.~Gruber},
\authitem{G.~Kalicy},
\authitem{R.~Karabowicz},
\authitem{R.~Kliemt},
\authitem{M.~Krebs},
\authitem{J.~Kunkel},
\authitem{U.~Kurilla},
\authitem{D.~Lehmann},
\authitem{S.~Löchner},
\authitem{J.~Lühning},
\authitem{U.~Lynen},
\authitem{H.~Orth},
\authitem{M.~Patsyuk},
\authitem{K.~Peters},
\authitem{N.~Saito},
\authitem{T.~Saito},
\authitem{G.~Schepers},
\authitem{C. J.~Schmidt},
\authitem{C.~Schwarz},
\authitem{J.~Schwiening},
\authitem{A.~Täschner},
\authitem{M.~Traxler},
\authitem{C.~Ugur},
\authitem{B.~Voss},
\authitem{P.~Wieczorek},
\authitem{A.~Wilms},
\authitem{M.~Zühlsdorf},
\authitem{M.~Zyzak}
\lastitem
\institem{Veksler-Baldin Laboratory of High Energies (VBLHE), Joint Institute for Nuclear Research,{ \bf Dubna}, Russia}
\authitem{V.~Abazov},
\authitem{G.~Alexeev},
\authitem{V. A.~Arefiev},
\authitem{V.~Astakhov},
\authitem{M. Yu.~Barabanov},
\authitem{B. V.~Batyunya},
\authitem{Y.~Davydov},
\authitem{V. Kh.~Dodokhov},
\authitem{A.~Efremov},
\authitem{A.~Fechtchenko},
\authitem{A. G.~Fedunov},
\authitem{A.~Galoyan},
\authitem{S.~Grigoryan},
\authitem{E. K.~Koshurnikov},
\authitem{Y. Yu.~Lobanov},
\authitem{V. I.~Lobanov},
\authitem{A. F.~Makarov},
\authitem{L. V.~Malinina},
\authitem{V.~Malyshev},
\authitem{A. G.~Olshevskiy},
\authitem{E.~Perevalova},
\authitem{A. A.~Piskun},
\authitem{T.~Pocheptsov},
\authitem{G.~Pontecorvo},
\authitem{V.~Rodionov},
\authitem{Y.~Rogov},
\authitem{R.~Salmin},
\authitem{A.~Samartsev},
\authitem{M. G.~Sapozhnikov},
\authitem{G.~Shabratova},
\authitem{N. B.~Skachkov},
\authitem{A. N.~Skachkova},
\authitem{E. A.~Strokovsky},
\authitem{M.~Suleimanov},
\authitem{R.~Teshev},
\authitem{V.~Tokmenin},
\authitem{V.~Uzhinsky},
\authitem{A.~Vodopianov},
\authitem{S. A.~Zaporozhets},
\authitem{N. I.~Zhuravlev},
\authitem{A. G.~Zorin}
\lastitem
\institem{University of Edinburgh,{ \bf Edinburgh}, United Kingdom}
\authitem{D.~Branford},
\authitem{D.~Glazier},
\authitem{D.~Watts},
\authitem{P.~Woods}
\lastitem
\institem{Friedrich Alexander Universität Erlangen-Nürnberg,{ \bf Erlangen}, Germany}
\authitem{M.~Böhm},
\authitem{A.~Britting},
\authitem{W.~Eyrich},
\authitem{A.~Lehmann},
\authitem{F.~Uhlig}
\lastitem
\institem{Northwestern University,{ \bf Evanston}, U.S.A.}
\authitem{S.~Dobbs},
\authitem{K.~Seth},
\authitem{A.~Tomaradze},
\authitem{T.~Xiao}
\lastitem
\institem{Università di Ferrara and INFN Sezione di Ferrara,{ \bf Ferrara}, Italy}
\authitem{D.~Bettoni},
\authitem{V.~Carassiti},
\authitem{A.~Cotta Ramusino},
\authitem{P.~Dalpiaz},
\authitem{A.~Drago},
\authitem{E.~Fioravanti},
\authitem{I.~Garzia},
\authitem{M.~Savrie},
\authitem{G.~Stancari}
\lastitem
\institem{Goethe Universität, Institut für Kernphysik,{ \bf Frankfurt}, Germany}
\authitem{V.~Akishina}
\lastitem
\institem{Frankfurt Institute for Advanced Studies,{ \bf Frankfurt}, Germany}
\authitem{E.~Iakovleva},
\authitem{I.~Kisel},
\authitem{G.~Kozlov},
\authitem{I.~Kulakov},
\authitem{M.~Pugach}
\lastitem
\institem{INFN Laboratori Nazionali di Frascati,{ \bf Frascati}, Italy}
\authitem{N.~Bianchi},
\authitem{P.~Gianotti},
\authitem{C.~Guaraldo},
\authitem{V.~Lucherini},
\authitem{D.~Orecchini},
\authitem{E.~Pace}
\lastitem
\institem{INFN Sezione di Genova,{ \bf Genova}, Italy}
\authitem{A.~Bersani},
\authitem{G.~Bracco},
\authitem{M.~Macri},
\authitem{R. F.~Parodi}
\lastitem
\institem{Justus Liebig-Universität Gießen II. Physikalisches Institut,{ \bf Gießen}, Germany}
\authitem{S.~Bianco},
\authitem{K.~Biguenko},
\authitem{D.~Bremer},
\authitem{K.~Brinkmann},
\authitem{V.~Di Pietro},
\authitem{S.~Diehl},
\authitem{V.~Dormenev},
\authitem{P.~Drexler},
\authitem{M.~Düren},
\authitem{T.~Eißner},
\authitem{E.~Etzelmüller},
\authitem{S.~Fleischer},
\authitem{K.~Föhl},
\authitem{M.~Galuska},
\authitem{T.~Geßler},
\authitem{E.~Gutz},
\authitem{C.~Hahn},
\authitem{A.~Hayrapetyan},
\authitem{M.~Kesselkaul},
\authitem{B.~Kröck},
\authitem{W.~Kühn},
\authitem{T.~Kuske},
\authitem{J. S.~Lange},
\authitem{Y.~Liang},
\authitem{O.~Merle},
\authitem{V.~Metag},
\authitem{D.~Mühlheim},
\authitem{D.~Münchow},
\authitem{M.~Nanova},
\authitem{S.~Nazarenko},
\authitem{R.~Novotny},
\authitem{A.~Pitka},
\authitem{T.~Quagli},
\authitem{S.~Reiter},
\authitem{J.~Rieke},
\authitem{C.~Rosenbaum},
\authitem{M.~Schmidt},
\authitem{R.~Schnell},
\authitem{B.~Spruck},
\authitem{H.~Stenzel},
\authitem{U.~Thöring},
\authitem{T.~Ullrich},
\authitem{M. N.~Wagner},
\authitem{T.~Wasem},
\authitem{M.~Werner},
\authitem{B.~Wohlfahrt},
\authitem{H.~Zaunick}
\lastitem
\institem{University of Glasgow,{ \bf Glasgow}, United Kingdom}
\authitem{D.~Ireland},
\authitem{G.~Rosner},
\authitem{B.~Seitz}
\lastitem
\institem{Birla Institute of Technology and Science - Pilani , K.K. Birla Goa Campus,{ \bf Goa}, India}
\authitem{P.N.~Deepak},
\authitem{A.~Kulkarni}
\lastitem
\institem{KVI-Center for Advanced Radiation Technology (CART), University of Groningen,{ \bf Groningen}, Netherlands}
\authitem{A.~Apostolou},
\authitem{M.~Babai},
\authitem{M.~Kavatsyuk},
\authitem{P. J.~Lemmens},
\authitem{M.~Lindemulder},
\authitem{H.~Loehner},
\authitem{J.~Messchendorp},
\authitem{P.~Schakel},
\authitem{H.~Smit},
\authitem{M.~Tiemens},
\authitem{J. C.~van der Weele},
\authitem{R.~Veenstra},
\authitem{S.~Vejdani}
\lastitem
\institem{Gauhati University, Physics Department,{ \bf Guwahati}, India}
\authitem{K.~Dutta},
\authitem{K.~Kalita}
\lastitem
\institem{Indian Institute of Technology Indore, School of Science,{ \bf Indore}, India}
\authitem{A.~Kumar},
\authitem{A.~Roy},
\authitem{R.~Sahoo}
\lastitem
\institem{Fachhochschule Südwestfalen,{ \bf Iserlohn}, Germany}
\authitem{H.~Sohlbach}
\lastitem
\institem{Forschungszentrum Jülich, Institut für Kernphysik,{ \bf Jülich}, Germany}
\authitem{L.~Bianchi},
\authitem{M.~Büscher},
\authitem{L.~Cao},
\authitem{A.~Cebulla},
\authitem{D.~Deermann},
\authitem{R.~Dosdall},
\authitem{S.~Esch},
\authitem{A.~Gillitzer},
\authitem{A.~Goerres},
\authitem{F.~Goldenbaum},
\authitem{D.~Grunwald},
\authitem{A.~Herten},
\authitem{Q.~Hu},
\authitem{G.~Kemmerling},
\authitem{H.~Kleines},
\authitem{A.~Lehrach},
\authitem{R.~Maier},
\authitem{R.~Nellen},
\authitem{H.~Ohannessian},
\authitem{H.~Ohm},
\authitem{S.~Orfanitski},
\authitem{D.~Prasuhn},
\authitem{E.~Prencipe},
\authitem{J.~Ritman},
\authitem{S.~Schadmand},
\authitem{J.~Schumann},
\authitem{T.~Sefzick},
\authitem{V.~Serdyuk},
\authitem{G.~Sterzenbach},
\authitem{T.~Stockmanns},
\authitem{P.~Wintz},
\authitem{P.~Wüstner},
\authitem{H.~Xu}
\lastitem
\institem{Chinese Academy of Science, Institute of Modern Physics,{ \bf Lanzhou}, China}
\authitem{S.~Li},
\authitem{Z.~Li},
\authitem{Z.~Sun},
\authitem{H.~Xu}
\lastitem
\institem{INFN Laboratori Nazionali di Legnaro,{ \bf Legnaro}, Italy}
\authitem{V.~Rigato}
\lastitem
\institem{Lunds Universitet, Department of Physics,{ \bf Lund}, Sweden}
\authitem{K.~Fissum},
\authitem{K.~Hansen},
\authitem{L.~Isaksson},
\authitem{M.~Lundin},
\authitem{B.~Schröder}
\lastitem
\institem{Johannes Gutenberg-Universität, Institut für Kernphysik,{ \bf Mainz}, Germany}
\authitem{P.~Achenbach},
\authitem{O.~Corell},
\authitem{A.~Denig},
\authitem{M.~Distler},
\authitem{M.~Hoek},
\authitem{A.~Karavdina},
\authitem{W.~Lauth},
\authitem{H.~Merkel},
\authitem{U.~Müller},
\authitem{J.~Pochodzalla},
\authitem{S.~Sanchez},
\authitem{S.~Schlimme},
\authitem{C.~Sfienti},
\authitem{M.~Thiel},
\authitem{M.~Zambrana},
\authitem{L.~Zhiqing}
\lastitem
\institem{Helmholtz-Institut Mainz,{ \bf Mainz}, Germany}
\authitem{H.~Ahmadi},
\authitem{S.~Ahmed },
\authitem{S.~Bleser},
\authitem{L.~Capozza},
\authitem{M.~Cardinali},
\authitem{A.~Dbeyssi},
\authitem{M.~Deiseroth},
\authitem{F.~Feldbauer},
\authitem{M.~Fritsch},
\authitem{B.~Fröhlich},
\authitem{P.~Jasinski},
\authitem{D.~Kang},
\authitem{D.~Khaneft},
\authitem{R.~Klasen},
\authitem{H. H.~Leithoff},
\authitem{D.~Lin},
\authitem{F.~Maas},
\authitem{S.~Maldaner},
\authitem{M.~Marta},
\authitem{M.~Michel},
\authitem{M. C.~Mora Espi},
\authitem{C.~Morales Morales},
\authitem{C.~Motzko},
\authitem{F.~Nerling},
\authitem{O.~Noll},
\authitem{S.~Pflüger},
\authitem{D.~Rodriguez Pineiro},
\authitem{A.~Sanchez-Lorente},
\authitem{M.~Steinen},
\authitem{R.~Valente},
\authitem{T.~Weber},
\authitem{I.~Zimmermann}
\lastitem
\institem{Research Institute for Nuclear Problems, Belarus State University,{ \bf Minsk}, Belarus}
\authitem{A.~Fedorov},
\authitem{M.~Korjik},
\authitem{O.~Missevitch}
\lastitem
\institem{Moscow Power Engineering Institute,{ \bf Moscow}, Russia}
\authitem{A.~Boukharov},
\authitem{O.~Malyshev},
\authitem{I.~Marishev},
\authitem{A.~Semenov}
\lastitem
\institem{Institute for Theoretical and Experimental Physics,{ \bf Moscow}, Russia}
\authitem{P.~Balanutsa},
\authitem{V.~Balanutsa},
\authitem{V.~Chernetsky},
\authitem{A.~Demekhin},
\authitem{A.~Dolgolenko},
\authitem{P.~Fedorets},
\authitem{A.~Gerasimov},
\authitem{V.~Goryachev}
\lastitem
\institem{Nuclear Physics Division, Bhabha Atomic Research Centre,{ \bf Mumbai}, India}
\authitem{V.~Chandratre},
\authitem{V.~Datar},
\authitem{D.~Dutta},
\authitem{V.~Jha},
\authitem{H.~Kumawat},
\authitem{A.K.~Mohanty},
\authitem{A.~Parmar},
\authitem{B.~Roy}
\lastitem
\institem{Indian Institute of Technology Bombay, Department of Physics,{ \bf Mumbai}, India}
\authitem{S.~Dash},
\authitem{M.~Jadhav},
\authitem{S.~Kumar},
\authitem{P.~Sarin},
\authitem{R.~Varma}
\lastitem
\institem{Technische Universität München,{ \bf München}, Germany}
\authitem{I.~Konorov},
\authitem{S.~Paul}
\lastitem
\institem{Westfälische Wilhelms-Universität Münster,{ \bf Münster}, Germany}
\authitem{S.~Grieser},
\authitem{A.~Hergemöller},
\authitem{B.~Hetz},
\authitem{A.~Khoukaz},
\authitem{E.~Köhler},
\authitem{J. P.~Wessels}
\lastitem
\institem{Suranaree University of Technology,{ \bf Nakhon Ratchasima}, Thailand}
\authitem{K.~Khosonthongkee},
\authitem{C.~Kobdaj},
\authitem{A.~Limphirat},
\authitem{P.~Srisawad},
\authitem{Y.~Yan}
\lastitem
\institem{Budker Institute of Nuclear Physics,{ \bf Novosibirsk}, Russia}
\authitem{M.~Barnyakov},
\authitem{A. Yu.~Barnyakov},
\authitem{K.~Beloborodov},
\authitem{V. E.~Blinov},
\authitem{A. E.~Blinov},
\authitem{V. S.~Bobrovnikov},
\authitem{S.~Kononov},
\authitem{E. A.~Kravchenko},
\authitem{I. A.~Kuyanov},
\authitem{K.~Martin},
\authitem{A. P.~Onuchin},
\authitem{S.~Serednyakov},
\authitem{A.~Sokolov},
\authitem{Y.~Tikhonov}
\lastitem
\institem{Institut de Physique Nucléaire dzOrsay (UMR8608), CNRS/IN2P3 and Université Paris-sud,{ \bf Orsay}, France}
\authitem{E.~Atomssa},
\authitem{T.~Hennino},
\authitem{M.~Imre},
\authitem{R.~Kunne},
\authitem{C.~Le Galliard},
\authitem{B.~Ma},
\authitem{D.~Marchand},
\authitem{S.~Ong},
\authitem{B.~Ramstein},
\authitem{P.~Rosier},
\authitem{J.~van de Wiele},
\authitem{Y.~Wang}
\lastitem
\institem{Dipartimento di Fisica, Università di Pavia, INFN Sezione di Pavia,{ \bf Pavia}, Italy}
\authitem{G.~Boca},
\authitem{S.~Costanza},
\authitem{P.~Genova},
\authitem{P.~Montagna},
\authitem{A.~Rotondi}
\lastitem
\institem{Institute for High Energy Physics,{ \bf Protvino}, Russia}
\authitem{V.~Abramov},
\authitem{N.~Belikov},
\authitem{S.~Bukreeva},
\authitem{A.~Davidenko},
\authitem{A.~Derevschikov},
\authitem{Y.~Goncharenko},
\authitem{V.~Grishin},
\authitem{V.~Kachanov},
\authitem{V.~Kormilitsin},
\authitem{A.~Levin},
\authitem{Y.~Melnik},
\authitem{N.~Minaev},
\authitem{V.~Mochalov},
\authitem{D.~Morozov},
\authitem{L.~Nogach},
\authitem{S.~Poslavskiy},
\authitem{A.~Ryazantsev},
\authitem{S.~Ryzhikov},
\authitem{P.~Semenov},
\authitem{I.~Shein},
\authitem{A.~Uzunian},
\authitem{A.~Vasiliev},
\authitem{A.~Yakutin}
\lastitem
\institem{IRFU,SPHN, CEA Saclay,{ \bf Saclay}, France}
\authitem{E.~Tomasi-Gustafsson}
\lastitem
\institem{Sikaha-Bhavana, Visva-Bharati, WB,{ \bf Santiniketan}, India}
\authitem{U.~Roy}
\lastitem
\institem{University of Sidney, School of Physics,{ \bf Sidney}, Australia}
\authitem{B.~Yabsley}
\lastitem
\institem{Petersburg Nuclear Physics Institute of Russian Academy of Science, Gatchina,{ \bf St. Petersburg}, Russia}
\authitem{S.~Belostotski},
\authitem{G.~Gavrilov},
\authitem{A.~Kashchuk},
\authitem{O.~Levitskaya},
\authitem{S.~Manaenkov},
\authitem{O.~Miklukho},
\authitem{Y.~Naryshkin},
\authitem{K.~Suvorov},
\authitem{D.~Veretennikov},
\authitem{A.~Zhdanov}
\lastitem
\institem{National Research Centre "Kurchatov Institute" B.P.KONSTANTINOV PETERSBURG NUCLEAR PHYSICS INSTITUTE, Gatchina,{ \bf St. Petersburg}, Russia}
\authitem{A.~Izotov}
\lastitem
\institem{Stockholms Universitet,{ \bf Stockholm}, Sweden}
\authitem{K.~Makonyi},
\authitem{P.~Tegner},
\authitem{K. M.~von Würtemberg},
\authitem{D.~Wölbing}
\lastitem
\institem{Kungliga Tekniska Högskolan,{ \bf Stockholm}, Sweden}
\authitem{T.~Bäck},
\authitem{B.~Cederwall}
\lastitem
\institem{Sardar Vallabhbhai National Institute of Technology, Applied Physics Department,{ \bf Surat}, India}
\authitem{A. K.~Rai}
\lastitem
\institem{Veer Narmad South Gujarat University, Department of Physics,{ \bf Surat}, India}
\authitem{S.~Godre}
\lastitem
\institem{Università di Torino and INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{A.~Amoroso},
\authitem{M. P.~Bussa},
\authitem{L.~Busso},
\authitem{F.~De Mori},
\authitem{M.~Destefanis},
\authitem{L.~Fava},
\authitem{L.~Ferrero},
\authitem{M.~Greco},
\authitem{J.~Hu},
\authitem{L.~Lavezzi},
\authitem{M.~Maggiora},
\authitem{G.~Maniscalco},
\authitem{S.~Marcello},
\authitem{S.~Sosio},
\authitem{S.~Spataro}
\lastitem
\institem{INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{D.~Calvo},
\authitem{S.~Coli},
\authitem{P.~De Remigis},
\authitem{A.~Filippi},
\authitem{G.~Giraudo},
\authitem{S.~Lusso},
\authitem{G.~Mazza},
\authitem{M.~Mignone},
\authitem{A.~Rivetti},
\authitem{R.~Wheadon},
\authitem{L.~Zotti}
\lastitem
\institem{Politecnico di Torino and INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{F.~Balestra},
\authitem{F.~Iazzi},
\authitem{R.~Introzzi},
\authitem{A.~Lavagno},
\authitem{J.~Olave},
\authitem{H.~Younis}
\lastitem
\institem{Università di Trieste and INFN Sezione di Trieste,{ \bf Trieste}, Italy}
\authitem{R.~Birsa},
\authitem{F.~Bradamante},
\authitem{A.~Bressan},
\authitem{A.~Martin}
\lastitem
\institem{Universität Tübingen,{ \bf Tübingen}, Germany}
\authitem{H.~Clement}
\lastitem
\institem{Uppsala Universitet, Institutionen för fysik och astronomi,{ \bf Uppsala}, Sweden}
\authitem{L.~Caldeira Balkestahl},
\authitem{H.~Calen},
\authitem{K.~Fransson},
\authitem{W.~Ikegami Andersson},
\authitem{T.~Johansson},
\authitem{A.~Kupsc},
\authitem{P.~Marciniewski},
\authitem{M.~Papenbrock},
\authitem{J.~Pettersson},
\authitem{K.~Schönning},
\authitem{M.~Wolke},
\authitem{J.~Zlomanczuk}
\lastitem
\institem{The Svedberg Laboratory,{ \bf Uppsala}, Sweden}
\authitem{B.~Galnander}
\lastitem
\institem{Universitat de Valencia Dpto. de Física Atómica, Molecular y Nuclear,{ \bf Valencia}, Spain}
\authitem{J.~Diaz}
\lastitem
\institem{Sardar Patel University, Physics Department,{ \bf Vallabh Vidynagar}, India}
\authitem{V.~Pothodi Chackara}
\lastitem
\institem{National Centre for Nuclear Research,{ \bf Warsaw}, Poland}
\authitem{A.~Chlopik},
\authitem{G.~Kesik},
\authitem{D.~Melnychuk},
\authitem{B.~Slowinski},
\authitem{A.~Trzcinski},
\authitem{M.~Wojciechowski},
\authitem{S.~Wronka},
\authitem{B.~Zwieglinski}
\lastitem
\institem{Österreichische Akademie der Wissenschaften, Stefan Meyer Institut für Subatomare Physik,{ \bf Wien}, Austria}
\authitem{S.~Brunner},
\authitem{P.~Bühler},
\authitem{J.~Marton},
\authitem{D.~Steinschaden},
\authitem{K.~Suzuki},
\authitem{E.~Widmann},
\authitem{J.~Zmeskal}
\lastitem


==> collaboration/PANDA-author-list-01-02-2016.tex <==
%
% PANDA Collaboration  - authorlist - automatically generated by PANDA website
2016-02-01 03:15:06\\[14pt] 
%
\institem{Aligarth Muslim University, Physics Department,{ \bf Aligarth}, India}
\authitem{B.~Singh}
\lastitem
\institem{Universität Basel,{ \bf Basel}, Switzerland}
\authitem{W.~Erni},
\authitem{B.~Krusche},
\authitem{M.~Steinacher},
\authitem{N.~Walford}
\lastitem
\institem{Institute of High Energy Physics, Chinese Academy of Sciences,{ \bf Beijing}, China}
\authitem{H.~Liu},
\authitem{Z.~Liu},
\authitem{B.~Liu},
\authitem{X.~Shen},
\authitem{C.~Wang},
\authitem{J.~Zhao}
\lastitem
\institem{Universität Bochum, Institut für Experimentalphysik I,{ \bf Bochum}, Germany}
\authitem{M.~Albrecht},
\authitem{T.~Erlen},
\authitem{M.~Fink},
\authitem{F.~Heinsius},
\authitem{T.~Held},
\authitem{T.~Holtmann},
\authitem{S.~Jasper},
\authitem{I.~Keshk},
\authitem{H.~Koch},
\authitem{B.~Kopf},
\authitem{M.~Kuhlmann},
\authitem{M.~Kümmel},
\authitem{S.~Leiber},
\authitem{M.~Mikirtychyants},
\authitem{P.~Musiol},
\authitem{A.~Mustafa},
\authitem{M.~Pelizäus},
\authitem{J.~Pychy},
\authitem{M.~Richter},
\authitem{C.~Schnier},
\authitem{T.~Schröder},
\authitem{C.~Sowa},
\authitem{M.~Steinke},
\authitem{T.~Triffterer},
\authitem{U.~Wiedner}
\lastitem
\institem{Rheinische Friedrich-Wilhelms-Universität Bonn,{ \bf Bonn}, Germany}
\authitem{M.~Ball},
\authitem{R.~Beck},
\authitem{C.~Hammann},
\authitem{B.~Ketzer},
\authitem{M.~Kube},
\authitem{P.~Mahlberg},
\authitem{M.~Rossbach},
\authitem{C.~Schmidt},
\authitem{R.~Schmitz},
\authitem{U.~Thoma},
\authitem{M.~Urban},
\authitem{D.~Walther},
\authitem{C.~Wendel},
\authitem{A.~Wilson}
\lastitem
\institem{Università di Brescia,{ \bf Brescia}, Italy}
\authitem{A.~Bianconi}
\lastitem
\institem{Institutul National de C\&D pentru Fizica si Inginerie Nucleara "Horia Hulubei",{ \bf Bukarest-Magurele}, Romania}
\authitem{M.~Bragadireanu},
\authitem{M.~Caprini},
\authitem{D.~Pantea}
\lastitem
\institem{P.D. Patel Institute of Applied Science, Department of Physical Sciences,{ \bf Changa}, India}
\authitem{B.~Patel}
\lastitem
\institem{University of Technology, Institute of Applied Informatics,{ \bf Cracow}, Poland}
\authitem{W.~Czyzycki},
\authitem{M.~Domagala},
\authitem{G.~Filo},
\authitem{J.~Jaworowski},
\authitem{M.~Krawczyk},
\authitem{E.~Lisowski},
\authitem{F.~Lisowski},
\authitem{M.~Michałek},
\authitem{P.~Poznański},
\authitem{J.~Płażek}
\lastitem
\institem{IFJ, Institute of Nuclear Physics PAN,{ \bf Cracow}, Poland}
\authitem{K.~Korcyl},
\authitem{A.~Kozela},
\authitem{P.~Kulessa},
\authitem{P.~Lebiedowicz},
\authitem{K.~Pysz},
\authitem{W.~Schäfer},
\authitem{A.~Szczurek}
\lastitem
\institem{AGH, University of Science and Technology,{ \bf Cracow}, Poland}
\authitem{T.~Fiutowski},
\authitem{M.~Idzik},
\authitem{B.~Mindur},
\authitem{D.~Przyborowski},
\authitem{K.~Swientek}
\lastitem
\institem{Instytut Fizyki, Uniwersytet Jagiellonski,{ \bf Cracow}, Poland}
\authitem{J.~Biernat},
\authitem{B.~Kamys},
\authitem{S.~Kistryn},
\authitem{G.~Korcyl},
\authitem{W.~Krzemien},
\authitem{A.~Magiera},
\authitem{P.~Moskal},
\authitem{A.~Pyszniak},
\authitem{Z.~Rudy},
\authitem{P.~Salabura},
\authitem{J.~Smyrski},
\authitem{P.~Strzempek},
\authitem{A.~Wronska}
\lastitem
\institem{FAIR, Facility for Antiproton and Ion Research in Europe,{ \bf Darmstadt}, Germany}
\authitem{I.~Augustin},
\authitem{R.~Böhm},
\authitem{I.~Lehmann},
\authitem{D.~Nicmorus Marinescu},
\authitem{L.~Schmitt},
\authitem{V.~Varentsov}
\lastitem
\institem{GSI Helmholtzzentrum für Schwerionenforschung GmbH,{ \bf Darmstadt}, Germany}
\authitem{M.~Al-Turany},
\authitem{A.~Belias},
\authitem{H.~Deppe},
\authitem{R.~Dzhygadlo},
\authitem{A.~Ehret},
\authitem{H.~Flemming},
\authitem{A.~Gerhardt},
\authitem{K.~Götzen},
\authitem{A.~Gromliuk},
\authitem{L.~Gruber},
\authitem{R.~Karabowicz},
\authitem{R.~Kliemt},
\authitem{M.~Krebs},
\authitem{U.~Kurilla},
\authitem{D.~Lehmann},
\authitem{S.~Löchner},
\authitem{J.~Lühning},
\authitem{U.~Lynen},
\authitem{H.~Orth},
\authitem{M.~Patsyuk},
\authitem{K.~Peters},
\authitem{T.~Saito},
\authitem{G.~Schepers},
\authitem{C. J.~Schmidt},
\authitem{C.~Schwarz},
\authitem{J.~Schwiening},
\authitem{A.~Täschner},
\authitem{M.~Traxler},
\authitem{C.~Ugur},
\authitem{B.~Voss},
\authitem{P.~Wieczorek},
\authitem{A.~Wilms},
\authitem{M.~Zühlsdorf}
\lastitem
\institem{Veksler-Baldin Laboratory of High Energies (VBLHE), Joint Institute for Nuclear Research,{ \bf Dubna}, Russia}
\authitem{V.~Abazov},
\authitem{G.~Alexeev},
\authitem{V. A.~Arefiev},
\authitem{V.~Astakhov},
\authitem{M. Yu.~Barabanov},
\authitem{B. V.~Batyunya},
\authitem{Y.~Davydov},
\authitem{V. Kh.~Dodokhov},
\authitem{A.~Efremov},
\authitem{A.~Fechtchenko},
\authitem{A. G.~Fedunov},
\authitem{A.~Galoyan},
\authitem{S.~Grigoryan},
\authitem{E. K.~Koshurnikov},
\authitem{Y. Yu.~Lobanov},
\authitem{V. I.~Lobanov},
\authitem{A. F.~Makarov},
\authitem{L. V.~Malinina},
\authitem{V.~Malyshev},
\authitem{A. G.~Olshevskiy},
\authitem{E.~Perevalova},
\authitem{A. A.~Piskun},
\authitem{T.~Pocheptsov},
\authitem{G.~Pontecorvo},
\authitem{V.~Rodionov},
\authitem{Y.~Rogov},
\authitem{R.~Salmin},
\authitem{A.~Samartsev},
\authitem{M. G.~Sapozhnikov},
\authitem{G.~Shabratova},
\authitem{N. B.~Skachkov},
\authitem{A. N.~Skachkova},
\authitem{E. A.~Strokovsky},
\authitem{M.~Suleimanov},
\authitem{R.~Teshev},
\authitem{V.~Tokmenin},
\authitem{V.~Uzhinsky},
\authitem{A.~Vodopianov},
\authitem{S. A.~Zaporozhets},
\authitem{N. I.~Zhuravlev},
\authitem{A. G.~Zorin}
\lastitem
\institem{University of Edinburgh,{ \bf Edinburgh}, United Kingdom}
\authitem{D.~Branford},
\authitem{D.~Glazier},
\authitem{D.~Watts}
\lastitem
\institem{Friedrich Alexander Universität Erlangen-Nürnberg,{ \bf Erlangen}, Germany}
\authitem{M.~Böhm},
\authitem{A.~Britting},
\authitem{W.~Eyrich},
\authitem{A.~Lehmann},
\authitem{F.~Uhlig}
\lastitem
\institem{Northwestern University,{ \bf Evanston}, U.S.A.}
\authitem{S.~Dobbs},
\authitem{K.~Seth},
\authitem{A.~Tomaradze},
\authitem{T.~Xiao}
\lastitem
\institem{Università di Ferrara and INFN Sezione di Ferrara,{ \bf Ferrara}, Italy}
\authitem{D.~Bettoni},
\authitem{V.~Carassiti},
\authitem{A.~Cotta Ramusino},
\authitem{P.~Dalpiaz},
\authitem{A.~Drago},
\authitem{E.~Fioravanti},
\authitem{I.~Garzia},
\authitem{M.~Savrie}
\lastitem
\institem{Frankfurt Institute for Advanced Studies,{ \bf Frankfurt}, Germany}
\authitem{V.~Akishina},
\authitem{I.~Kisel},
\authitem{G.~Kozlov},
\authitem{M.~Pugach},
\authitem{M.~Zyzak}
\lastitem
\institem{INFN Laboratori Nazionali di Frascati,{ \bf Frascati}, Italy}
\authitem{P.~Gianotti},
\authitem{C.~Guaraldo},
\authitem{V.~Lucherini}
\lastitem
\institem{INFN Sezione di Genova,{ \bf Genova}, Italy}
\authitem{A.~Bersani},
\authitem{G.~Bracco},
\authitem{M.~Macri},
\authitem{R. F.~Parodi}
\lastitem
\institem{Justus Liebig-Universität Gießen II. Physikalisches Institut,{ \bf Gießen}, Germany}
\authitem{K.~Biguenko},
\authitem{K.~Brinkmann},
\authitem{V.~Di Pietro},
\authitem{S.~Diehl},
\authitem{V.~Dormenev},
\authitem{P.~Drexler},
\authitem{M.~Düren},
\authitem{E.~Etzelmüller},
\authitem{M.~Galuska},
\authitem{E.~Gutz},
\authitem{C.~Hahn},
\authitem{A.~Hayrapetyan},
\authitem{M.~Kesselkaul},
\authitem{W.~Kühn},
\authitem{T.~Kuske},
\authitem{J. S.~Lange},
\authitem{Y.~Liang},
\authitem{O.~Merle},
\authitem{V.~Metag},
\authitem{M.~Nanova},
\authitem{S.~Nazarenko},
\authitem{R.~Novotny},
\authitem{T.~Quagli},
\authitem{S.~Reiter},
\authitem{J.~Rieke},
\authitem{C.~Rosenbaum},
\authitem{M.~Schmidt},
\authitem{R.~Schnell},
\authitem{H.~Stenzel},
\authitem{U.~Thöring},
\authitem{T.~Ullrich},
\authitem{M. N.~Wagner},
\authitem{T.~Wasem},
\authitem{B.~Wohlfahrt},
\authitem{H.~Zaunick}
\lastitem
\institem{University of Glasgow,{ \bf Glasgow}, United Kingdom}
\authitem{D.~Ireland},
\authitem{G.~Rosner},
\authitem{B.~Seitz}
\lastitem
\institem{Birla Institute of Technology and Science - Pilani , K.K. Birla Goa Campus,{ \bf Goa}, India}
\authitem{P.N.~Deepak},
\authitem{A.~Kulkarni}
\lastitem
\institem{KVI-Center for Advanced Radiation Technology (CART), University of Groningen,{ \bf Groningen}, Netherlands}
\authitem{A.~Apostolou},
\authitem{M.~Babai},
\authitem{M.~Kavatsyuk},
\authitem{P. J.~Lemmens},
\authitem{M.~Lindemulder},
\authitem{H.~Loehner},
\authitem{J.~Messchendorp},
\authitem{P.~Schakel},
\authitem{H.~Smit},
\authitem{M.~Tiemens},
\authitem{J. C.~van der Weele},
\authitem{R.~Veenstra},
\authitem{S.~Vejdani}
\lastitem
\institem{Gauhati University, Physics Department,{ \bf Guwahati}, India}
\authitem{K.~Dutta},
\authitem{K.~Kalita}
\lastitem
\institem{Indian Institute of Technology Indore, School of Science,{ \bf Indore}, India}
\authitem{A.~Kumar},
\authitem{A.~Roy}
\lastitem
\institem{Fachhochschule Südwestfalen,{ \bf Iserlohn}, Germany}
\authitem{H.~Sohlbach}
\lastitem
\institem{Forschungszentrum Jülich, Institut für Kernphysik,{ \bf Jülich}, Germany}
\authitem{M.~Bai},
\authitem{L.~Bianchi},
\authitem{M.~Büscher},
\authitem{L.~Cao},
\authitem{A.~Cebulla},
\authitem{R.~Dosdall},
\authitem{A.~Gillitzer},
\authitem{F.~Goldenbaum},
\authitem{D.~Grunwald},
\authitem{A.~Herten},
\authitem{Q.~Hu},
\authitem{G.~Kemmerling},
\authitem{H.~Kleines},
\authitem{A.~Lehrach},
\authitem{R.~Nellen},
\authitem{H.~Ohm},
\authitem{S.~Orfanitski},
\authitem{D.~Prasuhn},
\authitem{E.~Prencipe},
\authitem{J.~Ritman},
\authitem{S.~Schadmand},
\authitem{T.~Sefzick},
\authitem{V.~Serdyuk},
\authitem{G.~Sterzenbach},
\authitem{T.~Stockmanns},
\authitem{P.~Wintz},
\authitem{P.~Wüstner},
\authitem{H.~Xu},
\authitem{A.~Zambanini}
\lastitem
\institem{Chinese Academy of Science, Institute of Modern Physics,{ \bf Lanzhou}, China}
\authitem{S.~Li},
\authitem{Z.~Li},
\authitem{Z.~Sun},
\authitem{H.~Xu}
\lastitem
\institem{INFN Laboratori Nazionali di Legnaro,{ \bf Legnaro}, Italy}
\authitem{V.~Rigato}
\lastitem
\institem{Lunds Universitet, Department of Physics,{ \bf Lund}, Sweden}
\authitem{L.~Isaksson}
\lastitem
\institem{Johannes Gutenberg-Universität, Institut für Kernphysik,{ \bf Mainz}, Germany}
\authitem{P.~Achenbach},
\authitem{O.~Corell},
\authitem{A.~Denig},
\authitem{M.~Distler},
\authitem{M.~Hoek},
\authitem{A.~Karavdina},
\authitem{W.~Lauth},
\authitem{Z.~Liu},
\authitem{H.~Merkel},
\authitem{U.~Müller},
\authitem{J.~Pochodzalla},
\authitem{S.~Sanchez},
\authitem{S.~Schlimme},
\authitem{C.~Sfienti},
\authitem{M.~Thiel}
\lastitem
\institem{Helmholtz-Institut Mainz,{ \bf Mainz}, Germany}
\authitem{H.~Ahmadi},
\authitem{S.~Ahmed },
\authitem{S.~Bleser},
\authitem{L.~Capozza},
\authitem{M.~Cardinali},
\authitem{A.~Dbeyssi},
\authitem{M.~Deiseroth},
\authitem{F.~Feldbauer},
\authitem{M.~Fritsch},
\authitem{B.~Fröhlich},
\authitem{P.~Jasinski},
\authitem{D.~Kang},
\authitem{D.~Khaneft},
\authitem{R.~Klasen},
\authitem{H. H.~Leithoff},
\authitem{D.~Lin},
\authitem{F.~Maas},
\authitem{S.~Maldaner},
\authitem{M.~Marta},
\authitem{M.~Michel},
\authitem{M. C.~Mora Espí},
\authitem{C.~Morales Morales},
\authitem{C.~Motzko},
\authitem{F.~Nerling},
\authitem{O.~Noll},
\authitem{S.~Pflüger},
\authitem{A.~Pitka},
\authitem{D.~Rodríguez Piñeiro},
\authitem{A.~Sanchez-Lorente},
\authitem{M.~Steinen},
\authitem{R.~Valente},
\authitem{T.~Weber},
\authitem{M.~Zambrana},
\authitem{I.~Zimmermann}
\lastitem
\institem{Research Institute for Nuclear Problems, Belarus State University,{ \bf Minsk}, Belarus}
\authitem{A.~Fedorov},
\authitem{M.~Korjik},
\authitem{O.~Missevitch}
\lastitem
\institem{Moscow Power Engineering Institute,{ \bf Moscow}, Russia}
\authitem{A.~Boukharov},
\authitem{O.~Malyshev},
\authitem{I.~Marishev}
\lastitem
\institem{Institute for Theoretical and Experimental Physics,{ \bf Moscow}, Russia}
\authitem{P.~Balanutsa},
\authitem{V.~Balanutsa},
\authitem{V.~Chernetsky},
\authitem{A.~Demekhin},
\authitem{A.~Dolgolenko},
\authitem{P.~Fedorets},
\authitem{A.~Gerasimov},
\authitem{V.~Goryachev}
\lastitem
\institem{Nuclear Physics Division, Bhabha Atomic Research Centre,{ \bf Mumbai}, India}
\authitem{V.~Chandratre},
\authitem{V.~Datar},
\authitem{D.~Dutta},
\authitem{V.~Jha},
\authitem{H.~Kumawat},
\authitem{A.K.~Mohanty},
\authitem{A.~Parmar},
\authitem{B.~Roy},
\authitem{G.~Sonika}
\lastitem
\institem{Indian Institute of Technology Bombay, Department of Physics,{ \bf Mumbai}, India}
\authitem{S.~Dash},
\authitem{M.~Jadhav},
\authitem{S.~Kumar},
\authitem{P.~Sarin},
\authitem{R.~Varma}
\lastitem
\institem{Westfälische Wilhelms-Universität Münster,{ \bf Münster}, Germany}
\authitem{S.~Grieser},
\authitem{A.~Hergemöller},
\authitem{B.~Hetz},
\authitem{A.~Khoukaz},
\authitem{J. P.~Wessels}
\lastitem
\institem{Suranaree University of Technology,{ \bf Nakhon Ratchasima}, Thailand}
\authitem{K.~Khosonthongkee},
\authitem{C.~Kobdaj},
\authitem{A.~Limphirat},
\authitem{P.~Srisawad},
\authitem{Y.~Yan}
\lastitem
\institem{Budker Institute of Nuclear Physics,{ \bf Novosibirsk}, Russia}
\authitem{M.~Barnyakov},
\authitem{A. Yu.~Barnyakov},
\authitem{K.~Beloborodov},
\authitem{A. E.~Blinov},
\authitem{V. E.~Blinov},
\authitem{V. S.~Bobrovnikov},
\authitem{S.~Kononov},
\authitem{E. A.~Kravchenko},
\authitem{I. A.~Kuyanov},
\authitem{K.~Martin},
\authitem{A. P.~Onuchin},
\authitem{S.~Serednyakov},
\authitem{A.~Sokolov},
\authitem{Y.~Tikhonov}
\lastitem
\institem{Institut de Physique Nucléaire, CNRS-IN2P3, Univ. Paris-Sud, Université Paris-Saclay, 91406,{ \bf Orsay cedex}, France}
\authitem{E.~Atomssa},
\authitem{R.~Kunne},
\authitem{D.~Marchand},
\authitem{B.~Ramstein},
\authitem{J.~van de Wiele},
\authitem{Y.~Wang}
\lastitem
\institem{Dipartimento di Fisica, Università di Pavia, INFN Sezione di Pavia,{ \bf Pavia}, Italy}
\authitem{G.~Boca},
\authitem{S.~Costanza},
\authitem{P.~Genova},
\authitem{P.~Montagna},
\authitem{A.~Rotondi}
\lastitem
\institem{Institute for High Energy Physics,{ \bf Protvino}, Russia}
\authitem{V.~Abramov},
\authitem{N.~Belikov},
\authitem{S.~Bukreeva},
\authitem{A.~Davidenko},
\authitem{A.~Derevschikov},
\authitem{Y.~Goncharenko},
\authitem{V.~Grishin},
\authitem{V.~Kachanov},
\authitem{V.~Kormilitsin},
\authitem{A.~Levin},
\authitem{Y.~Melnik},
\authitem{N.~Minaev},
\authitem{V.~Mochalov},
\authitem{D.~Morozov},
\authitem{L.~Nogach},
\authitem{S.~Poslavskiy},
\authitem{A.~Ryazantsev},
\authitem{S.~Ryzhikov},
\authitem{P.~Semenov},
\authitem{I.~Shein},
\authitem{A.~Uzunian},
\authitem{A.~Vasiliev},
\authitem{A.~Yakutin}
\lastitem
\institem{IRFU,SPHN, CEA Saclay,{ \bf Saclay}, France}
\authitem{E.~Tomasi-Gustafsson}
\lastitem
\institem{Sikaha-Bhavana, Visva-Bharati, WB,{ \bf Santiniketan}, India}
\authitem{U.~Roy}
\lastitem
\institem{University of Sidney, School of Physics,{ \bf Sidney}, Australia}
\authitem{B.~Yabsley}
\lastitem
\institem{National Research Centre "Kurchatov Institute" B.P.KONSTANTINOV PETERSBURG NUCLEAR PHYSICS INSTITUTE, Gatchina,{ \bf St. Petersburg}, Russia}
\authitem{S.~Belostotski},
\authitem{G.~Gavrilov},
\authitem{A.~Izotov},
\authitem{S.~Manaenkov},
\authitem{O.~Miklukho},
\authitem{D.~Veretennikov},
\authitem{A.~Zhdanov}
\lastitem
\institem{Petersburg Nuclear Physics Institute of Russian Academy of Science, Gatchina,{ \bf St. Petersburg}, Russia}
\authitem{A.~Kashchuk},
\authitem{O.~Levitskaya},
\authitem{Y.~Naryshkin},
\authitem{K.~Suvorov}
\lastitem
\institem{Stockholms Universitet,{ \bf Stockholm}, Sweden}
\authitem{K.~Makonyi},
\authitem{M.~Preston},
\authitem{P.~Tegner},
\authitem{D.~Wölbing}
\lastitem
\institem{Kungliga Tekniska Högskolan,{ \bf Stockholm}, Sweden}
\authitem{T.~Bäck},
\authitem{B.~Cederwall}
\lastitem
\institem{Sardar Vallabhbhai National Institute of Technology, Applied Physics Department,{ \bf Surat}, India}
\authitem{A. K.~Rai}
\lastitem
\institem{Veer Narmad South Gujarat University, Department of Physics,{ \bf Surat}, India}
\authitem{S.~Godre}
\lastitem
\institem{INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{D.~Calvo},
\authitem{S.~Coli},
\authitem{P.~De Remigis},
\authitem{A.~Filippi},
\authitem{G.~Giraudo},
\authitem{S.~Lusso},
\authitem{G.~Mazza},
\authitem{M.~Mignone},
\authitem{A.~Rivetti},
\authitem{R.~Wheadon}
\lastitem
\institem{Università di Torino and INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{A.~Amoroso},
\authitem{M. P.~Bussa},
\authitem{L.~Busso},
\authitem{F.~De Mori},
\authitem{M.~Destefanis},
\authitem{L.~Fava},
\authitem{L.~Ferrero},
\authitem{M.~Greco},
\authitem{J.~Hu},
\authitem{L.~Lavezzi},
\authitem{M.~Maggiora},
\authitem{G.~Maniscalco},
\authitem{S.~Marcello},
\authitem{S.~Sosio},
\authitem{S.~Spataro}
\lastitem
\institem{Politecnico di Torino and INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{F.~Balestra},
\authitem{F.~Iazzi},
\authitem{R.~Introzzi},
\authitem{A.~Lavagno},
\authitem{J.~Olave}
\lastitem
\institem{Università di Trieste and INFN Sezione di Trieste,{ \bf Trieste}, Italy}
\authitem{R.~Birsa},
\authitem{F.~Bradamante},
\authitem{A.~Bressan},
\authitem{A.~Martin}
\lastitem
\institem{Uppsala Universitet, Institutionen för fysik och astronomi,{ \bf Uppsala}, Sweden}
\authitem{H.~Calen},
\authitem{W.~Ikegami Andersson},
\authitem{T.~Johansson},
\authitem{A.~Kupsc},
\authitem{P.~Marciniewski},
\authitem{M.~Papenbrock},
\authitem{J.~Pettersson},
\authitem{K.~Schönning},
\authitem{M.~Wolke}
\lastitem
\institem{The Svedberg Laboratory,{ \bf Uppsala}, Sweden}
\authitem{B.~Galnander}
\lastitem
\institem{Instituto de F\'{i}sica Corpuscular, Universidad de Valencia-CSIC,{ \bf Valencia}, Spain}
\authitem{J.~Diaz}
\lastitem
\institem{Sardar Patel University, Physics Department,{ \bf Vallabh Vidynagar}, India}
\authitem{V.~Pothodi Chackara}
\lastitem
\institem{National Centre for Nuclear Research,{ \bf Warsaw}, Poland}
\authitem{A.~Chlopik},
\authitem{G.~Kesik},
\authitem{D.~Melnychuk},
\authitem{B.~Slowinski},
\authitem{A.~Trzcinski},
\authitem{M.~Wojciechowski},
\authitem{S.~Wronka},
\authitem{B.~Zwieglinski}
\lastitem
\institem{Österreichische Akademie der Wissenschaften, Stefan Meyer Institut für Subatomare Physik,{ \bf Wien}, Austria}
\authitem{P.~Bühler},
\authitem{J.~Marton},
\authitem{D.~Steinschaden},
\authitem{K.~Suzuki},
\authitem{E.~Widmann},
\authitem{J.~Zmeskal}
\lastitem


==> collaboration/PANDA-author-list.tex <==
%
% Panda TDR - Framework
%
%\documentclass[pdftex]{panda_book}
%\documentclass[pdftex]
%\documentclass[12pt]{article}
\usepackage{hyperref}
\usepackage[utf8]{inputenc}
\usepackage{polski}
\usepackage[polish]{babel}

\RequirePackage{xspace}
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\lastitem{\vspace{0.5cm}\\ }%
\def\respitem#1{\institem{{\bf #1}\lastitem\\}}%
\let\groupitem=\authitem
%
\def\PANDA{\texorpdfstring{$\overline{\mbox{\sf P}}${\sf ANDA}}{Panda}\xspace}%
\def\Panda{\texorpdfstring{$\overline{\mbox{\sf P}}${\sf ANDA}}{Panda}\xspace}%
%
%\def\INST#1{\texorpdfstring{{\sf #1}}{{#1}}\xspace}%
%
%
\setlength{\topmargin}{-0.5cm}
\usepackage{anysize}
%\marginsize{left}{right}{top}{bottom}
\marginsize{2cm}{2cm}{1cm}{1cm}

%\textwidth 16cm
%
%
\begin{document}
%
\onecolumn
% 
\begin{center}
\vspace*{3mm }
{\LARGE The \Panda{} Collaboration}
%{\LARGE The Panda Collaboration}
\vskip 7mm
\input{authors}
\end{center}%
%
\end{document}
%

% EOF



==> collaboration/Panda_authors_list_actual.tex <==
% 
%PANDA Collaboration - authorlist - last updated: July 2012 by H.L\"ohner, KVI
% ordered alphaberically according to city name of affiliation
%
\institem{Universit\"at Basel, {\bf Basel}, Switzerland}
\authitem{W.~Erni},
\authitem{I.~Keshelashvili},
\authitem{B.~Krusche},
\authitem{M.~Steinacher}\lastitem
%
\institem{Institute of High Energy Physics, Chinese Academy of Sciences, {\bf Beijing}, China}
\authitem{Y.~Heng},
\authitem{Z.~Liu},
\authitem{H.~Liu},
\authitem{X.~Shen},
\authitem{Q.~Wang},
\authitem{H.~Xu}\lastitem
%
\institem{I. Institut f\"ur Experimentalphysik, Ruhr-Universit\"at Bochum, {\bf Bochum},  Germany}
\authitem{A.~Aab},
\authitem{M.~Albrecht},
\authitem{J.~Becker},
\authitem{A.~Csap\'o},
\authitem{F.~Feldbauer},
\authitem{M.~Fink},
\authitem{P.~Friedel},
\authitem{F.H.~Heinsius},
\authitem{T.~Held},
\authitem{L.~Klask},
\authitem{H.~Koch},
\authitem{B.~Kopf},
\authitem{S.~Leiber},
\authitem{M.~Leyhe},
\authitem{C.~Motzko},
\authitem{M.~Peliz\"aus},
\authitem{J.~Pychy},
\authitem{B.~Roth},
\authitem{T.~Schr\"oder},
\authitem{J.~Schulze},
\authitem{C.~Sowa},
\authitem{M.~Steinke},
\authitem{T.~Trifterer},
\authitem{U.~Wiedner},
\authitem{J.~Zhong}\lastitem
%
\institem{I. Institut f\"ur Experimentalphysik, Rheinische Friedrich Wilhelms-Universit\"at Bonn, {\bf Bonn}, Germany}
\authitem{R.~Beck},
\authitem{S.~Bianco},
\authitem{C.~Hammann},
\authitem{F.~Hinterberger},
\authitem{D.~Kaiser},
\authitem{M.~Kube},
\authitem{C.~Schmidt},
\authitem{R.~Schmitz},
\authitem{U.~Thoma},
\authitem{D.~Walther},
\authitem{C.~Wendel},
\authitem{T.~W\"urschig},
\authitem{H.G.~Zaunick}\lastitem
%
\institem{Universit\`{a}~di Brescia, {\bf Brescia}, Italy}
\authitem{A.~Bianconi}\lastitem
%
\institem{Institutul National de C\&D pentru Fizica si Inginerie Nucleara ``Horia Hulubei", {\bf Bukarest-Magurele}, Romania}
\authitem{M.~Bragadireanu},
\authitem{M.~Caprini},
\authitem{D.~Pantea},
\authitem{D.~Pantelica},
\authitem{D.~Pietreanu},
\authitem{L.~Serbina},
\authitem{P.D.~Tarta}\lastitem
%
\institem{Illinois Institute of Technology, {\bf Chicago}, USA}
\authitem{D.~Kaplan}\lastitem
%
\institem{FAIR - Facility for Antiproton and Ion Research in Europe, {\bf Darmstadt}, Germany}
\authitem{I.~Augustin},
\authitem{I.~Lehmann},
\authitem{D.~Nicmorus},
\authitem{G.~Schepers},
\authitem{L.~Schmitt}\lastitem
%
\institem{GSI Helmholtzzentrum für Schwerionenforschung GmbH, {\bf Darmstadt}, Germany}
\authitem{M.~Al-Turany},
\authitem{R.~Arora},
\authitem{H.~Deppe},
\authitem{H.~Flemming},
\authitem{A.~Gerhardt},
\authitem{K.~G\"otzen},
\authitem{G.~Kalicy},
\authitem{R.~Karabowicz},
\authitem{R.~Kliemt},
\authitem{D.~Lehmann},
\authitem{B.~Lewandowski},
\authitem{J.~L\"uhning},
\authitem{F.~Maas},
\authitem{H.~Orth},
\authitem{M.~Patsyuk},
\authitem{K.~Peters},
\authitem{T.~Saito},
\authitem{C.J.~Schmidt},
\authitem{C.~Schwarz},
\authitem{J.~Schwiening},
\authitem{B.~Voss},
\authitem{P.~Wieczorek},
\authitem{A.~Wilms},
\authitem{M.~Z\"uhlsdorf}\lastitem
%
\institem{Joint Institute for Nuclear Research, {\bf Dubna},
Russia}
\authitem{V.M.~Abazov}, 
\authitem{G.D.~Alexeev},
\authitem{V.A.~Arefiev},
\authitem{V.I.~Astakhov},
\authitem{M.Yu.~Barabanov},
\authitem{B.V.~Batyunya},
\authitem{Yu.I.~Davydov},
\authitem{V.Kh.~Dodokhov},
\authitem{A.A.~Efremov},
\authitem{A.G.~Fedunov},
\authitem{A.A.~Festchenko}, 
\authitem{A.S.~Galoyan},
\authitem{S.~Grigoryan},
\authitem{A.~Karmokov},
\authitem{E.K.~Koshurnikov},
\authitem{V.I.~Lobanov},
\authitem{Yu.Yu.~Lobanov},
\authitem{A.F.~Makarov},
\authitem{L.V.~Malinina},
\authitem{V.L.~Malyshev},
\authitem{G.A.~Mustafaev},
\authitem{A.G.~Olshevski},
\authitem{M.A.~Pasyuk},
\authitem{E.A.~Perevalova},
\authitem{A.A.~Piskun},
\authitem{T.A.~Pocheptsov},
\authitem{G.~Pontecorvo},
\authitem{V.K.~Rodionov},
\authitem{Yu.N.~Rogov},
\authitem{R.A.~Salmin},
\authitem{A.G.~Samartsev},
\authitem{M.G.~Sapozhnikov},
\authitem{G.S.~Shabratova},
\authitem{N.B.~Skachkov}, 
\authitem{A.N.~Skachkova}, 
\authitem{E.A.~Strokovsky},
\authitem{M.K.~Suleimanov},
\authitem{R.Sh.~Teshev},
\authitem{V.V.~Tokmenin},
\authitem{V.V.~Uzhinsky}
\authitem{A.S.~Vodopyanov},
\authitem{S.A.~Zaporozhets},
\authitem{N.I.~Zhuravlev},
\authitem{A.G.~Zorin}\lastitem
%
\institem{University of Edinburgh, {\bf Edinburgh}, United Kingdom}
\authitem{D.~Branford},
\authitem{D.~Glazier},
\authitem{D.~Watts},
\authitem{P.~Woods}\lastitem
%
\institem{Friedrich Alexander Universit\"at Erlangen-N\"urnberg, {\bf Erlangen-N\"urnberg}, Germany}
\authitem{A.~Britting},
\authitem{W.~Eyrich},
\authitem{A.~Lehmann},
\authitem{F.~Uhlig}\lastitem
%
\institem{Northwestern University, {\bf Evanston}, USA}
\authitem{S.~Dobbs},
\authitem{Z.~Metreveli},
\authitem{K.~Seth},
\authitem{A.~Tomaradze},
\authitem{T.~Xiao}\lastitem
%
\institem{Universit\`{a} di Ferrara and INFN Sezione di Ferrara, {\bf Ferrara}, Italy}
\authitem{D.~Bettoni},
\authitem{V.~Carassiti},
\authitem{A.~Cotta Ramusino},
\authitem{P.~Dalpiaz},
\authitem{A.~Drago},
\authitem{E.~Fioravanti},
\authitem{I.~Garzia},
\authitem{M.~Savri\`e},
\authitem{G.~Stancari}\lastitem
%
\institem{INFN Laboratori Nazionali di Frascati, {\bf Frascati}, Italy}
\authitem{N.~Bianchi},
\authitem{P.~Gianotti},
\authitem{C.~Guaraldo},
\authitem{V.~Lucherini},
\authitem{D.~Orecchini},
\authitem{E.~Pace}\lastitem
%
\institem{INFN Sezione di Genova, {\bf Genova}, Italy}
\authitem{A.~Bersani},
\authitem{G.~Bracco},
\authitem{M.~Macri},
\authitem{R.F.~Parodi}\lastitem
%
\institem{II. Physikalisches Institut, Justus Liebig-Universit\"at Gie\ss{}en, {\bf Gie\ss{}en}, Germany}
\authitem{D.~Bremer},
\authitem{K.T.~Brinkmann}, 
\authitem{V.~Dormenev},
\authitem{P.~Drexler}, 
\authitem{M.~D\"uren},
\authitem{T.~Ei\ss{}ner},
\authitem{K.~F\"ohl},
\authitem{M.~Galuska},
\authitem{T.~Ge\ss{}ler},
\authitem{A.~Hayrapetyan},
\authitem{J.~Hu},
\authitem{P.~Koch},
\authitem{B.~Kr\"ock},
\authitem{W.~K\"uhn},
\authitem{S.~Lange},
\authitem{Y.~Liang},
\authitem{O.~Merle},
\authitem{V.~Metag},
\authitem{M.~Moritz},
\authitem{D.~M\"unchow},
\authitem{M.~Nanova}, 
\authitem{R.~Novotny},
\authitem{A.~Pitka},
\authitem{T.~Quagli},
\authitem{R.~Schnell},
\authitem{B.~Spruck},
\authitem{H.~Stenzel},
\authitem{T.~Ullrich},
\authitem{M.~Werner},
\authitem{H.~Xu}\lastitem
%
\institem{University of Glasgow, {\bf Glasgow}, United Kingdom}
\authitem{C.~Euan},
\authitem{M.~Hoek},
\authitem{D.~Ireland},
\authitem{T.~Keri},
\authitem{R.~Montgomery},
\authitem{D.~Protopopescu},
\authitem{G.~Rosner},
\authitem{B.~Seitz}\lastitem
%
\institem{Kernfysisch Versneller Instituut, University of Groningen, {\bf Groningen}, Netherlands}
\authitem{M.~Babai},
\authitem{A.~Glazenborg-Kluttig},
\authitem{M.~Kavatsyuk},
\authitem{P.~Lemmens},
\authitem{M.~Lindemulder},
\authitem{H.~L\"ohner},
\authitem{J.~Messchendorp},
\authitem{H.~Moeini},
\authitem{P.~Schakel},
\authitem{F.~Schreuder},
\authitem{H.~Smit},
\authitem{G.~Tambave},
\authitem{J.C.~van der Weele},
\authitem{R.~Veenstra}\lastitem
%
\institem{Fachhochschule S\"udwestfalen, {\bf Iserlohn}, Germany}
\authitem{H.~Sohlbach}\lastitem
%
\institem{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, {\bf J\"ulich}, Germany}
\authitem{M.~B\"uscher},
\authitem{D.~Deermann},
\authitem{R.~Dosdall},
\authitem{S.~Esch},
\authitem{A.~Gillitzer},
\authitem{A.~Goerres},
\authitem{F.~Goldenbaum},
\authitem{D.~Grunwald},
\authitem{S.~Henssler},
\authitem{A.~Herten},
\authitem{Q.~Hu},
\authitem{G.~Kemmerling},
\authitem{H.~Kleines},
\authitem{V.~Kozlov},
\authitem{A.~Lehrach},
\authitem{R.~Maier},
\authitem{M.~Mertens},
\authitem{R.~Nellen},
\authitem{H.~Ohm},
\authitem{S.~Orfanitski},
\authitem{N.~Paul},
\authitem{D.~Prasuhn},
\authitem{T.~Randriamalala},
\authitem{J.~Ritman},
\authitem{S.~Schadmand},
\authitem{T.~Sefzick},
\authitem{V.~Serdyuk},
\authitem{G.~Sterzenbach},
\authitem{T.~Stockmanns},
\authitem{P.~Wintz},
\authitem{P.~W\"ustner},
\authitem{H.~Xu}\lastitem
%
\institem{University of Silesia, {\bf Katowice}, Poland}
\authitem{J.~Kisiel}\lastitem
%
\institem{AGH University of Science and Technology, {\bf Krakow}, Poland}
\authitem{T.~Fiutowski},
\authitem{M.~Idzik},
\authitem{B.~Mindur},
\authitem{D.~Przyborowski},
\authitem{K.~Swientek}\lastitem
%
\institem{IFJ, Institute of Nuclear Physics PAN, {\bf Krakow}, Poland}
\authitem{B.~Czech},
\authitem{S.~Kliczewski},
\authitem{K.~Korcyl},
\authitem{A.~Kozela},
\authitem{P.~Kulessa},
\authitem{P.~Lebiedowicz},
\authitem{K.~Malgorzata},
\authitem{K.~Pysz},
\authitem{W.~Sch\"afer},
\authitem{R.~Siudak},
\authitem{A.~Szczurek}\lastitem
%
\institem{Instytut Fizyki, Uniwersytet Jagiellonski, {\bf Krakow}, Poland}
\authitem{J.~Biernat},
\authitem{S.~Jowzaee},
\authitem{B.~Kamys},
\authitem{S.~Kistryn},
\authitem{G.~Korcyl},
\authitem{W.~Krzemie\~n},
\authitem{A.~Magiera},
\authitem{P.~Moskal},
\authitem{M.~Pa\l ka},
\authitem{Z.~Rudy},
\authitem{P.~Salabura},
\authitem{J.~Smyrski},
\authitem{P.~Strzempek},
\authitem{A.~Wro\~nska}\lastitem
%
\institem{University Krakow, {\bf Krakow}, Poland}
\authitem{P.~Brandys},
\authitem{T.~Czyzewski},
\authitem{W.~Czyzycki},
\authitem{M.~Domagala},
\authitem{G.~Filo},
\authitem{M.~Hawryluk},
\authitem{M.~Krawczyk},
\authitem{D.~Kwiatkowski},
\authitem{E.~Lisowski},
\authitem{F.~Lisowski}\lastitem
%
\institem{Institute of Modern Physics, Chinese Academy of Science, {\bf Lanzhou}, China}
\authitem{S.~Li},
\authitem{Z.~Li},
\authitem{Z.~Sun},
\authitem{H.~Xu}\lastitem
%
\institem{INFN Laboratori Nazionali di Legnaro, {\bf Legnaro}, Italy}
\authitem{V.~Rigato}\lastitem
%
\institem{Department of Physics, Lunds Universitet, {\bf Lund}, Sweden}
\authitem{K.~Fissum},
\authitem{K.~Hansen},
\authitem{L.~Isaksson},
\authitem{M.~Lundin},
\authitem{B.~Schr\"oder}\lastitem
%
\institem{Institut f\"ur Kernphysik, Johannes Gutenberg-Universit\"at Mainz, {\bf Mainz}, Germany}
\authitem{P.~Achenbach},
\authitem{S.~Bleser},
\authitem{U.~Cahit},
\authitem{M.~Cardinali},
\authitem{A.~Denig},
\authitem{M.~Distler},
\authitem{M.~Fritsch},
\authitem{D.~Kangh},
\authitem{A.~Karavdina},
\authitem{W.~Lauth},
\authitem{H.~Merkel},
\authitem{M.~Michel},
\authitem{M.C.~Mora Espi},
\authitem{U.~M\"uller},
\authitem{J.~Pochodzalla},
\authitem{J.~Prometeusz},
\authitem{S.~Sanchez},
\authitem{A.~Sanchez-Lorente},
\authitem{S.~Schlimme},
\authitem{C.~Sfienti},
\authitem{M.~Steinen},
\authitem{M.~Thiel},
\authitem{T.~Weber}\lastitem
%
\institem{Research Institute for Nuclear Problems, Belarus State University, {\bf Minsk}, Belarus}
\authitem{V.I.~Dormenev},
\authitem{A.A.~Fedorov},
\authitem{M.V.~Korzhik},
\authitem{O.V.~Missevitch}\lastitem
%
\institem{Institute for Theoretical and Experimental Physics, {\bf Moscow}, Russia}
\authitem{V.~Balanutsa},
\authitem{V.~Chernetsky},
\authitem{A.~Demekhin},
\authitem{A.~Dolgolenko},
\authitem{P.~Fedorets},
\authitem{A.~Gerasimov},
\authitem{V.~Goryachev},
\authitem{V.~Varentsov}\lastitem
%
\institem{Moscow Power Engineering Institute, {\bf Moscow}, Russia}
\authitem{A.~Boukharov},
\authitem{O.~Malyshev},
\authitem{I.~Marishev},
\authitem{A.~Semenov}\lastitem
%
\institem{Department of Physics, Indian Institute of Technology Bombay, {\bf Mumbai}, India}
\authitem{R.~Varma}\lastitem
%
\institem{Bhabha Atomic Research Centre, Trombay, {\bf Mumbai}, India}
\authitem{A.~Chaterjee},
\authitem{V.~Jha},
\authitem{S.~Kailas},
\authitem{B.~Roy}\lastitem
%
\institem{Technische Universit\"at {\bf M\"unchen}, Germany}
\authitem{F.~B\"ohmer},
\authitem{S.~D$\o$rheim},
\authitem{B.~Ketzer},
\authitem{I.~Konorov},
\authitem{S.~Paul}\lastitem
%
\institem{Westf\"alische Wilhelms-Universit\"at {\bf M\"unster}, Germany}
\authitem{A.K.~Hergem\"oller},
\authitem{A.~Khoukaz},
\authitem{E.~K\"ohler},
\authitem{A.~T\"aschner},
\authitem{J.~Wessels}\lastitem
%
\institem{Suranaree University of Technology, {\bf Nakhon Ratchasima}, Thailand}
\authitem{L.~Ayut},
\authitem{K.~Chinorat},
\authitem{K.~Khanchai},
\authitem{S.~Pornrad},
\authitem{Y.~Yan}\lastitem
%
\institem{Budker Institute of Nuclear Physics of Russian Academy of Science, {\bf Novosibirsk}, Russia}
\authitem{E.~Baldin},
\authitem{K.~Kotov},
\authitem{S.~Peleganchuk},
\authitem{Yu.~Tikhonov}\lastitem
%
\institem{Institut de Physique Nucl\'{e}aire, {\bf Orsay}, France}
\authitem{J.~Boucher},
\authitem{V.~Chambert},
\authitem{A.~Dbeyssi},
\authitem{T.~Hennino},
\authitem{M.~Imre}
\authitem{R.~Kunne},
\authitem{C.~Le~Galliard},
\authitem{B.~Ma},
\authitem{D.~Marchand},
\authitem{A.~Maroni},
\authitem{S.~Ong},
\authitem{B.~Ramstein},
\authitem{P.~Rosier},
\authitem{M.~Sudol},
\authitem{E.~Tomasi-Gustafsson},
\authitem{J.~Van~de~Wiele}\lastitem
%
\institem{Dipartimento di Fisica Nucleare e Teorica, Universit\`{a} di Pavia, 
INFN Sezione di Pavia, {\bf Pavia}, Italy}
\authitem{G.~Boca},
\authitem{A.~Braghieri},
\authitem{S.~Costanza},
\authitem{P.~Genova},
\authitem{L.~Lavezzi},
\authitem{P.~Montagna},
\authitem{A.~Rotondi}\lastitem
%
\institem{Institute for High Energy Physics, {\bf Protvino}, Russia}
\authitem{V.~Abramov},
\authitem{N.I.~Belikov},
\authitem{A.M.~Davidenko},
\authitem{A.A.~Derevschikov}, 
\authitem{Y.M.~Goncharenko},
\authitem{V.N.~Grishin}, 
\authitem{V.A.~Kachanov},
\authitem{D.A.~Konstantinov}, 
\authitem{V.A.~Kormilitsin},
\authitem{A.~Levin},
\authitem{Y.M.~Melnik},
\authitem{N.G.~Minaev}, 
\authitem{V.V.~Mochalov}, 
\authitem{D.A.~Morozov}, 
\authitem{L.V.~Nogach}, 
\authitem{S.~Poslavskiy}, 
\authitem{A.V.~Ryazantsev},
\authitem{S.~Ryzhikov},
\authitem{P.A.~Semenov},
\authitem{I.~Shein},
\authitem{A.V.~Uzunian},
\authitem{A.N.~Vasiliev},
\authitem{A.E.~Yakutin}\lastitem
%
\institem{Petersburg Nuclear Physics Institute of Russian Academy of Science,
Gatchina, {\bf St.~Petersburg}, Russia}
\authitem{S.~Belostotski},
\authitem{G.~Gavrilov},
\authitem{A.~Itzotov},
\authitem{A.~Kashchuk},
\authitem{A.~Kisselev},
\authitem{P.~Kravchenko},
\authitem{O.~Levitskaya},
\authitem{S.~Manaenkov},
\authitem{O.~Miklukho},
\authitem{Y.~Naryshkin},
\authitem{D.~Veretennikov},
\authitem{V.~Vikhrov},
\authitem{A.~Zhadanov}\lastitem
%
\institem{Stockholms Universitet, {\bf Stockholm}, Sweden}
\authitem{K.~Mak\'onyi},
\authitem{P.E.~Tegn\'{e}r},
\authitem{K.M.~von~W\"urtemberg}\lastitem
%
\institem{Kungliga Tekniska H\"ogskolan, {\bf Stockholm}, Sweden}
\authitem{T.~B\"ack},
\authitem{B.~Cederwall}\lastitem
%
\institem{INFN Sezione di Torino, {\bf Torino}, Italy}
\authitem{D.~Calvo},
\authitem{S.~Coli},
\authitem{P.~De~Remigis},
\authitem{A.~Filippi},
\authitem{G.~Giraudo},
\authitem{S.~Lusso},
\authitem{G.~Mazza},
\authitem{A.~Rivetti},
\authitem{R.~Wheadon}\lastitem
%
\institem{Politecnico di Torino and INFN Sezione di Torino, {\bf Torino}, Italy}
\authitem{F.~Iazzi},
\authitem{A.~Lavagno},
\authitem{H.~Younis}\lastitem
%
\institem{Universit\`{a} del Piemonte Orientale and INFN Sezione di Torino, {\bf Torino}, Italy}
\authitem{L. Fava}\lastitem
%
\institem{Universit\`{a} di Torino and INFN Sezione di Torino, {\bf Torino}, Italy}
\authitem{A.~Amoroso},
\authitem{M.P.~Bussa},
\authitem{L.~Busso}, 
\authitem{F.~De Mori},
\authitem{M.~Destefanis},
\authitem{L.~Ferrero},
\authitem{M.~Greco}, 
\authitem{M.~Maggiora},
\authitem{S.~Marcello},
\authitem{S.~Sosio},
\authitem{S.~Spataro},
\authitem{L.~Zotti}\lastitem
%
\institem{Universit\`{a} di Trieste and INFN Sezione di Trieste, {\bf Trieste}, Italy}
\authitem{R.~Birsa},
\authitem{F.~Bradamante},
\authitem{A.~Bressan},
\authitem{A.~Martin}\lastitem
%
\institem{Eberhard Karls-Universit\"at T\"ubingen, {\bf T\"ubingen}, Germany}
\authitem{H.~Clement}\lastitem
%
\institem{Institutionen f\"or fysik oct astronomi, Uppsala Universitet, {\bf Uppsala}, Sweden}
\authitem{L.~Caldeira Balkest{\aa}hl},
\authitem{H.~Cal\'en},
\authitem{K.~Fransson},
\authitem{T.~Johansson},
\authitem{A.~Kupsc},
\authitem{P.~Marciniewski},
\authitem{E.~Thom\'e},
\authitem{M.~Wolke},
\authitem{J.~Zlomanczuk}\lastitem
%
\institem{The Svedberg Laboratory, {\bf Uppsala}, Sweden}
\authitem{B.~G{\aa}lnander}\lastitem
%
\institem{Dpto. de F\'isica At\'omica, Molecular y Nuclear, Universitat de Valencia, {\bf Valencia}, Spain}
\authitem{J.~D\'iaz},
\authitem{A.~Ortiz}\lastitem
%
%
\institem{National Centre for Nuclear Research, {\bf Warsaw}, Poland}
\authitem{A.~Chlopik},
\authitem{Z.~Guzik},
\authitem{K.~Kosinski},
\authitem{D.~Melnychuk},
\authitem{B.~Slowinski},
\authitem{A.~Wasilewski},
\authitem{M.~Wojciechowski},
\authitem{S.~Wronka},
\authitem{A.~Wysocka},
\authitem{B.~Zwieglinski}\lastitem
%
\institem{Warsaw University of Technology, {\bf Warsaw}, Poland}
\authitem{J.~Bzdak},
\authitem{P.~Duda},
\authitem{A.~Pacan},
\authitem{B.~Slowinski}\lastitem
%
\institem{Stefan Meyer Institut f\"ur Subatomare Physik, \"Osterreichische Akademie der Wissenschaften, {\bf Wien}, Austria}
\authitem{P.~B\"uhler},
\authitem{O.~Hartman},
\authitem{P.~Kienle},
\authitem{J.~Marton},
\authitem{K.~Suzuki},
\authitem{E.~Widmann},
\authitem{J.~Zmeskal}\lastitem
%
%
\vspace{1cm}
{\bf last updated: August 1, 2012 by H. L\"ohner according to Memberlist 2012-05-07 from U.W. and recent CB-member response}\\
{\bf last updated: April 24, 2013 by U. Kurilla: Added 3 members of Jag. Uni. according to Jim's email}
%
%\centerline{$^\dagger$\ Membership to be approved by the Coordination Board}
%
% EOF
%


==> collaboration/authors_sep2016.tex <==
%
% PANDA Collaboration  - authorlist - automatically generated by PANDA website
2016-05-17 12:04:11 
%
\institem{Aligarth Muslim University, Physics Department,{ \bf Aligarth}, India}
\authitem{B.~Singh}
\lastitem
\institem{Universität Basel,{ \bf Basel}, Switzerland}
\authitem{W.~Erni},
\authitem{B.~Krusche},
\authitem{M.~Steinacher},
\authitem{N.~Walford}
\lastitem
\institem{Institute of High Energy Physics, Chinese Academy of Sciences,{ \bf Beijing}, China}
\authitem{B.~Liu},
\authitem{H.~Liu},
\authitem{Z.~Liu},
\authitem{X.~Shen},
\authitem{C.~Wang},
\authitem{J.~Zhao}
\lastitem
\institem{Universität Bochum, Institut für Experimentalphysik I,{ \bf Bochum}, Germany}
\authitem{M.~Albrecht},
\authitem{T.~Erlen},
\authitem{M.~Fink},
\authitem{F.~Heinsius},
\authitem{T.~Held},
\authitem{T.~Holtmann},
\authitem{S.~Jasper},
\authitem{I.~Keshk},
\authitem{H.~Koch},
\authitem{B.~Kopf},
\authitem{M.~Kuhlmann},
\authitem{M.~Kümmel},
\authitem{S.~Leiber},
\authitem{M.~Mikirtychyants},
\authitem{P.~Musiol},
\authitem{A.~Mustafa},
\authitem{M.~Pelizäus},
\authitem{J.~Pychy},
\authitem{M.~Richter},
\authitem{C.~Schnier},
\authitem{T.~Schröder},
\authitem{C.~Sowa},
\authitem{M.~Steinke},
\authitem{T.~Triffterer},
\authitem{U.~Wiedner}
\lastitem
\institem{Rheinische Friedrich-Wilhelms-Universität Bonn,{ \bf Bonn}, Germany}
\authitem{M.~Ball},
\authitem{R.~Beck},
\authitem{C.~Hammann},
\authitem{B.~Ketzer},
\authitem{M.~Kube},
\authitem{P.~Mahlberg},
\authitem{M.~Rossbach},
\authitem{C.~Schmidt},
\authitem{R.~Schmitz},
\authitem{U.~Thoma},
\authitem{M.~Urban},
\authitem{D.~Walther},
\authitem{C.~Wendel},
\authitem{A.~Wilson}
\lastitem
\institem{Università di Brescia,{ \bf Brescia}, Italy}
\authitem{A.~Bianconi}
\lastitem
\institem{Institutul National de C\&D pentru Fizica si Inginerie Nucleara "Horia Hulubei",{ \bf Bukarest-Magurele}, Romania}
\authitem{M.~Bragadireanu},
\authitem{M.~Caprini},
\authitem{D.~Pantea}
\lastitem
\institem{P.D. Patel Institute of Applied Science, Department of Physical Sciences,{ \bf Changa}, India}
\authitem{B.~Patel}
\lastitem
\institem{University of Technology, Institute of Applied Informatics,{ \bf Cracow}, Poland}
\authitem{W.~Czyzycki},
\authitem{M.~Domagala},
\authitem{G.~Filo},
\authitem{J.~Jaworowski},
\authitem{M.~Krawczyk},
\authitem{E.~Lisowski},
\authitem{F.~Lisowski},
\authitem{M.~Michałek},
\authitem{P.~Poznański},
\authitem{J.~Płażek}
\lastitem
\institem{IFJ, Institute of Nuclear Physics PAN,{ \bf Cracow}, Poland}
\authitem{K.~Korcyl},
\authitem{A.~Kozela},
\authitem{P.~Kulessa},
\authitem{P.~Lebiedowicz},
\authitem{K.~Pysz},
\authitem{W.~Schäfer},
\authitem{A.~Szczurek}
\lastitem
\institem{AGH, University of Science and Technology,{ \bf Cracow}, Poland}
\authitem{T.~Fiutowski},
\authitem{M.~Idzik},
\authitem{B.~Mindur},
\authitem{D.~Przyborowski},
\authitem{K.~Swientek}
\lastitem
\institem{Instytut Fizyki, Uniwersytet Jagiellonski,{ \bf Cracow}, Poland}
\authitem{J.~Biernat},
\authitem{B.~Kamys},
\authitem{S.~Kistryn},
\authitem{G.~Korcyl},
\authitem{W.~Krzemien},
\authitem{A.~Magiera},
\authitem{P.~Moskal},
\authitem{A.~Pyszniak},
\authitem{Z.~Rudy},
\authitem{P.~Salabura},
\authitem{J.~Smyrski},
\authitem{P.~Strzempek},
\authitem{A.~Wronska}
\lastitem
\institem{FAIR, Facility for Antiproton and Ion Research in Europe,{ \bf Darmstadt}, Germany}
\authitem{I.~Augustin},
\authitem{R.~Böhm},
\authitem{I.~Lehmann},
\authitem{D.~Nicmorus Marinescu},
\authitem{L.~Schmitt},
\authitem{V.~Varentsov}
\lastitem
\institem{GSI Helmholtzzentrum für Schwerionenforschung GmbH,{ \bf Darmstadt}, Germany}
\authitem{M.~Al-Turany},
\authitem{A.~Belias},
\authitem{H.~Deppe},
\authitem{R.~Dzhygadlo},
\authitem{A.~Ehret},
\authitem{H.~Flemming},
\authitem{A.~Gerhardt},
\authitem{K.~Götzen},
\authitem{A.~Gromliuk},
\authitem{L.~Gruber},
\authitem{R.~Hohler},
\authitem{G.~Kalicy},
\authitem{R.~Karabowicz},
\authitem{R.~Kliemt},
\authitem{M.~Krebs},
\authitem{U.~Kurilla},
\authitem{D.~Lehmann},
\authitem{S.~Löchner},
\authitem{J.~Lühning},
\authitem{U.~Lynen},
\authitem{H.~Orth},
\authitem{M.~Patsyuk},
\authitem{K.~Peters},
\authitem{T.~Saito},
\authitem{G.~Schepers},
\authitem{C. J.~Schmidt},
\authitem{C.~Schwarz},
\authitem{J.~Schwiening},
\authitem{A.~Täschner},
\authitem{M.~Traxler},
\authitem{C.~Ugur},
\authitem{B.~Voss},
\authitem{P.~Wieczorek},
\authitem{A.~Wilms},
\authitem{M.~Zühlsdorf}
\lastitem
\institem{Veksler-Baldin Laboratory of High Energies (VBLHE), Joint Institute for Nuclear Research,{ \bf Dubna}, Russia}
\authitem{V.~Abazov},
\authitem{G.~Alexeev},
\authitem{V. A.~Arefiev},
\authitem{V.~Astakhov},
\authitem{M. Yu.~Barabanov},
\authitem{B. V.~Batyunya},
\authitem{Y.~Davydov},
\authitem{V. Kh.~Dodokhov},
\authitem{A.~Efremov},
\authitem{A.~Fechtchenko},
\authitem{A. G.~Fedunov},
\authitem{A.~Galoyan},
\authitem{S.~Grigoryan},
\authitem{E. K.~Koshurnikov},
\authitem{Y. Yu.~Lobanov},
\authitem{V. I.~Lobanov},
\authitem{A. F.~Makarov},
\authitem{L. V.~Malinina},
\authitem{V.~Malyshev},
\authitem{A. G.~Olshevskiy},
\authitem{E.~Perevalova},
\authitem{A. A.~Piskun},
\authitem{T.~Pocheptsov},
\authitem{G.~Pontecorvo},
\authitem{V.~Rodionov},
\authitem{Y.~Rogov},
\authitem{R.~Salmin},
\authitem{A.~Samartsev},
\authitem{M. G.~Sapozhnikov},
\authitem{G.~Shabratova},
\authitem{N. B.~Skachkov},
\authitem{A. N.~Skachkova},
\authitem{E. A.~Strokovsky},
\authitem{M.~Suleimanov},
\authitem{R.~Teshev},
\authitem{V.~Tokmenin},
\authitem{V.~Uzhinsky},
\authitem{A.~Vodopianov},
\authitem{S. A.~Zaporozhets},
\authitem{N. I.~Zhuravlev},
\authitem{A. G.~Zorin}
\lastitem
\institem{University of Edinburgh,{ \bf Edinburgh}, United Kingdom}
\authitem{D.~Branford},
\authitem{D.~Glazier},
\authitem{D.~Watts}
\lastitem
\institem{Friedrich Alexander Universität Erlangen-Nürnberg,{ \bf Erlangen}, Germany}
\authitem{M.~Böhm},
\authitem{A.~Britting},
\authitem{W.~Eyrich},
\authitem{A.~Lehmann},
\authitem{M.~Pfaffinger},
\authitem{F.~Uhlig}
\lastitem
\institem{Northwestern University,{ \bf Evanston}, U.S.A.}
\authitem{S.~Dobbs},
\authitem{K.~Seth},
\authitem{A.~Tomaradze},
\authitem{T.~Xiao}
\lastitem
\institem{Università di Ferrara and INFN Sezione di Ferrara,{ \bf Ferrara}, Italy}
\authitem{D.~Bettoni},
\authitem{V.~Carassiti},
\authitem{A.~Cotta Ramusino},
\authitem{P.~Dalpiaz},
\authitem{A.~Drago},
\authitem{E.~Fioravanti},
\authitem{I.~Garzia},
\authitem{M.~Savrie}
\lastitem
\institem{Frankfurt Institute for Advanced Studies,{ \bf Frankfurt}, Germany}
\authitem{V.~Akishina},
\authitem{I.~Kisel},
\authitem{G.~Kozlov},
\authitem{M.~Pugach},
\authitem{M.~Zyzak}
\lastitem
\institem{INFN Laboratori Nazionali di Frascati,{ \bf Frascati}, Italy}
\authitem{P.~Gianotti},
\authitem{C.~Guaraldo},
\authitem{V.~Lucherini}
\lastitem
\institem{INFN Sezione di Genova,{ \bf Genova}, Italy}
\authitem{A.~Bersani},
\authitem{G.~Bracco},
\authitem{M.~Macri},
\authitem{R. F.~Parodi}
\lastitem
\institem{Justus Liebig-Universität Gießen II. Physikalisches Institut,{ \bf Gießen}, Germany}
\authitem{K.~Biguenko},
\authitem{K.~Brinkmann},
\authitem{V.~Di Pietro},
\authitem{S.~Diehl},
\authitem{V.~Dormenev},
\authitem{P.~Drexler},
\authitem{M.~Düren},
\authitem{E.~Etzelmüller},
%js added Klaus
\authitem{K.~Föhl},
\authitem{M.~Galuska},
\authitem{E.~Gutz},
\authitem{C.~Hahn},
\authitem{A.~Hayrapetyan},
\authitem{M.~Kesselkaul},
\authitem{W.~Kühn},
\authitem{T.~Kuske},
\authitem{J. S.~Lange},
\authitem{Y.~Liang},
\authitem{V.~Metag},
\authitem{M.~Nanova},
\authitem{S.~Nazarenko},
\authitem{R.~Novotny},
\authitem{T.~Quagli},
\authitem{S.~Reiter},
\authitem{A.~Riccardi},
\authitem{J.~Rieke},
\authitem{C.~Rosenbaum},
\authitem{M.~Schmidt},
\authitem{R.~Schnell},
\authitem{H.~Stenzel},
\authitem{U.~Thöring},
\authitem{T.~Ullrich},
\authitem{M. N.~Wagner},
\authitem{T.~Wasem},
\authitem{B.~Wohlfahrt},
\authitem{H.~Zaunick}
\lastitem
\institem{University of Glasgow,{ \bf Glasgow}, United Kingdom}
\authitem{D.~Ireland},
\authitem{G.~Rosner},
\authitem{B.~Seitz}
\lastitem
\institem{Birla Institute of Technology and Science - Pilani , K.K. Birla Goa Campus,{ \bf Goa}, India}
\authitem{P.N.~Deepak},
\authitem{A.~Kulkarni}
\lastitem
\institem{KVI-Center for Advanced Radiation Technology (CART), University of Groningen,{ \bf Groningen}, Netherlands}
\authitem{A.~Apostolou},
\authitem{M.~Babai},
\authitem{M.~Kavatsyuk},
\authitem{P. J.~Lemmens},
\authitem{M.~Lindemulder},
\authitem{H.~Loehner},
\authitem{J.~Messchendorp},
\authitem{P.~Schakel},
\authitem{H.~Smit},
\authitem{M.~Tiemens},
\authitem{J. C.~van der Weele},
\authitem{R.~Veenstra},
\authitem{S.~Vejdani}
\lastitem
\institem{Gauhati University, Physics Department,{ \bf Guwahati}, India}
\authitem{K.~Dutta},
\authitem{K.~Kalita}
\lastitem
\institem{Indian Institute of Technology Indore, School of Science,{ \bf Indore}, India}
\authitem{A.~Kumar},
\authitem{A.~Roy}
\lastitem
\institem{Fachhochschule Südwestfalen,{ \bf Iserlohn}, Germany}
\authitem{H.~Sohlbach}
\lastitem
\institem{Forschungszentrum Jülich, Institut für Kernphysik,{ \bf Jülich}, Germany}
\authitem{M.~Bai},
\authitem{L.~Bianchi},
\authitem{M.~Büscher},
\authitem{L.~Cao},
\authitem{A.~Cebulla},
\authitem{R.~Dosdall},
\authitem{A.~Gillitzer},
\authitem{F.~Goldenbaum},
\authitem{D.~Grunwald},
\authitem{A.~Herten},
\authitem{Q.~Hu},
\authitem{G.~Kemmerling},
\authitem{H.~Kleines},
\authitem{A.~Lehrach},
\authitem{R.~Nellen},
\authitem{H.~Ohm},
\authitem{S.~Orfanitski},
\authitem{D.~Prasuhn},
\authitem{E.~Prencipe},
\authitem{J.~Pütz},
\authitem{J.~Ritman},
\authitem{S.~Schadmand},
\authitem{T.~Sefzick},
\authitem{V.~Serdyuk},
\authitem{G.~Sterzenbach},
\authitem{T.~Stockmanns},
\authitem{P.~Wintz},
\authitem{P.~Wüstner},
\authitem{H.~Xu},
\authitem{A.~Zambanini}
\lastitem
\institem{Chinese Academy of Science, Institute of Modern Physics,{ \bf Lanzhou}, China}
\authitem{Z.~Li},
\authitem{S.~Li},
\authitem{Z.~Sun},
\authitem{H.~Xu}
\lastitem
\institem{INFN Laboratori Nazionali di Legnaro,{ \bf Legnaro}, Italy}
\authitem{V.~Rigato}
\lastitem
\institem{Lunds Universitet, Department of Physics,{ \bf Lund}, Sweden}
\authitem{L.~Isaksson}
\lastitem
\institem{Johannes Gutenberg-Universität, Institut für Kernphysik,{ \bf Mainz}, Germany}
\authitem{P.~Achenbach},
\authitem{O.~Corell},
\authitem{A.~Denig},
\authitem{M.~Distler},
\authitem{M.~Hoek},
\authitem{A.~Karavdina},
\authitem{W.~Lauth},
\authitem{Z.~Liu},
\authitem{H.~Merkel},
\authitem{U.~Müller},
\authitem{J.~Pochodzalla},
\authitem{S.~Sanchez},
\authitem{S.~Schlimme},
\authitem{C.~Sfienti},
\authitem{M.~Thiel}
\lastitem
\institem{Helmholtz-Institut Mainz,{ \bf Mainz}, Germany}
\authitem{H.~Ahmadi},
\authitem{S.~Ahmed },
\authitem{S.~Bleser},
\authitem{L.~Capozza},
\authitem{M.~Cardinali},
\authitem{A.~Dbeyssi},
\authitem{M.~Deiseroth},
\authitem{F.~Feldbauer},
\authitem{M.~Fritsch},
\authitem{B.~Fröhlich},
\authitem{P.~Jasinski},
\authitem{D.~Kang},
\authitem{D.~Khaneft},
\authitem{R.~Klasen},
\authitem{H. H.~Leithoff},
\authitem{D.~Lin},
\authitem{F.~Maas},
\authitem{S.~Maldaner},
\authitem{M.~Martínez},
\authitem{M.~Michel},
\authitem{M. C.~Mora Espí},
\authitem{C.~Morales Morales},
\authitem{C.~Motzko},
\authitem{F.~Nerling},
\authitem{O.~Noll},
\authitem{S.~Pflüger},
\authitem{A.~Pitka},
\authitem{D.~Rodríguez Piñeiro},
\authitem{A.~Sanchez-Lorente},
\authitem{M.~Steinen},
\authitem{R.~Valente},
\authitem{T.~Weber},
\authitem{M.~Zambrana},
\authitem{I.~Zimmermann}
\lastitem
\institem{Research Institute for Nuclear Problems, Belarus State University,{ \bf Minsk}, Belarus}
\authitem{A.~Fedorov},
\authitem{M.~Korjik},
\authitem{O.~Missevitch}
\lastitem
\institem{Moscow Power Engineering Institute,{ \bf Moscow}, Russia}
\authitem{A.~Boukharov},
\authitem{O.~Malyshev},
\authitem{I.~Marishev}
\lastitem
\institem{Institute for Theoretical and Experimental Physics,{ \bf Moscow}, Russia}
\authitem{V.~Balanutsa},
\authitem{P.~Balanutsa},
\authitem{V.~Chernetsky},
\authitem{A.~Demekhin},
\authitem{A.~Dolgolenko},
\authitem{P.~Fedorets},
\authitem{A.~Gerasimov},
\authitem{V.~Goryachev}
\lastitem
\institem{Nuclear Physics Division, Bhabha Atomic Research Centre,{ \bf Mumbai}, India}
\authitem{V.~Chandratre},
\authitem{V.~Datar},
\authitem{D.~Dutta},
\authitem{V.~Jha},
\authitem{H.~Kumawat},
\authitem{A.K.~Mohanty},
\authitem{A.~Parmar},
\authitem{B.~Roy},
\authitem{G.~Sonika}
\lastitem
\institem{Westfälische Wilhelms-Universität Münster,{ \bf Münster}, Germany}
\authitem{C.~Fritzsch},
\authitem{S.~Grieser},
\authitem{A.~Hergemöller},
\authitem{B.~Hetz},
\authitem{N.~Hüsken},
\authitem{A.~Khoukaz},
\authitem{J. P.~Wessels}
\lastitem
\institem{Suranaree University of Technology,{ \bf Nakhon Ratchasima}, Thailand}
\authitem{K.~Khosonthongkee},
\authitem{C.~Kobdaj},
\authitem{A.~Limphirat},
\authitem{P.~Srisawad},
\authitem{Y.~Yan}
\lastitem
\institem{Budker Institute of Nuclear Physics,{ \bf Novosibirsk}, Russia}
\authitem{M.~Barnyakov},
\authitem{A. Yu.~Barnyakov},
\authitem{K.~Beloborodov},
\authitem{A. E.~Blinov},
\authitem{V. E.~Blinov},
\authitem{V. S.~Bobrovnikov},
\authitem{S.~Kononov},
\authitem{E. A.~Kravchenko},
\authitem{I. A.~Kuyanov},
\authitem{K.~Martin},
\authitem{A. P.~Onuchin},
\authitem{S.~Serednyakov},
\authitem{A.~Sokolov},
\authitem{Y.~Tikhonov}
\lastitem
\institem{Institut de Physique Nucléaire, CNRS-IN2P3, Univ. Paris-Sud, Université Paris-Saclay, 91406,{ \bf Orsay cedex}, France}
\authitem{E.~Atomssa},
\authitem{R.~Kunne},
\authitem{D.~Marchand},
\authitem{B.~Ramstein},
\authitem{J.~van de Wiele},
\authitem{Y.~Wang}
\lastitem
\institem{Dipartimento di Fisica, Università di Pavia, INFN Sezione di Pavia,{ \bf Pavia}, Italy}
\authitem{G.~Boca},
\authitem{S.~Costanza},
\authitem{P.~Genova},
\authitem{P.~Montagna},
\authitem{A.~Rotondi}
\lastitem
\institem{Institute for High Energy Physics,{ \bf Protvino}, Russia}
\authitem{V.~Abramov},
\authitem{N.~Belikov},
\authitem{S.~Bukreeva},
\authitem{A.~Davidenko},
\authitem{A.~Derevschikov},
\authitem{Y.~Goncharenko},
\authitem{V.~Grishin},
\authitem{V.~Kachanov},
\authitem{V.~Kormilitsin},
\authitem{A.~Levin},
\authitem{Y.~Melnik},
\authitem{N.~Minaev},
\authitem{V.~Mochalov},
\authitem{D.~Morozov},
\authitem{L.~Nogach},
\authitem{S.~Poslavskiy},
\authitem{A.~Ryazantsev},
\authitem{S.~Ryzhikov},
\authitem{P.~Semenov},
\authitem{I.~Shein},
\authitem{A.~Uzunian},
\authitem{A.~Vasiliev},
\authitem{A.~Yakutin}
\lastitem
\institem{IRFU,SPHN, CEA Saclay,{ \bf Saclay}, France}
\authitem{E.~Tomasi-Gustafsson}
\lastitem
\institem{Sikaha-Bhavana, Visva-Bharati, WB,{ \bf Santiniketan}, India}
\authitem{U.~Roy}
\lastitem
\institem{University of Sidney, School of Physics,{ \bf Sidney}, Australia}
\authitem{B.~Yabsley}
\lastitem
\institem{National Research Centre "Kurchatov Institute" B.P.KONSTANTINOV PETERSBURG NUCLEAR PHYSICS INSTITUTE, Gatchina,{ \bf St. Petersburg}, Russia}
\authitem{S.~Belostotski},
\authitem{G.~Gavrilov},
\authitem{A.~Izotov},
\authitem{S.~Manaenkov},
\authitem{O.~Miklukho},
\authitem{D.~Veretennikov},
\authitem{A.~Zhdanov}
\lastitem
\institem{Stockholms Universitet,{ \bf Stockholm}, Sweden}
\authitem{K.~Makonyi},
\authitem{M.~Preston},
\authitem{P.~Tegner},
\authitem{D.~Wölbing}
\lastitem
\institem{Kungliga Tekniska Högskolan,{ \bf Stockholm}, Sweden}
\authitem{T.~Bäck},
\authitem{B.~Cederwall}
\lastitem
\institem{Sardar Vallabhbhai National Institute of Technology, Applied Physics Department,{ \bf Surat}, India}
\authitem{A. K.~Rai}
\lastitem
\institem{Veer Narmad South Gujarat University, Department of Physics,{ \bf Surat}, India}
\authitem{S.~Godre}
\lastitem
\institem{INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{D.~Calvo},
\authitem{S.~Coli},
\authitem{P.~De Remigis},
\authitem{A.~Filippi},
\authitem{G.~Giraudo},
\authitem{S.~Lusso},
\authitem{G.~Mazza},
\authitem{M.~Mignone},
\authitem{A.~Rivetti},
\authitem{R.~Wheadon}
\lastitem
\institem{Politecnico di Torino and INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{F.~Balestra},
\authitem{F.~Iazzi},
\authitem{R.~Introzzi},
\authitem{A.~Lavagno},
\authitem{J.~Olave}
\lastitem
\institem{Università di Torino and INFN Sezione di Torino,{ \bf Torino}, Italy}
\authitem{A.~Amoroso},
\authitem{M. P.~Bussa},
\authitem{L.~Busso},
\authitem{F.~De Mori},
\authitem{M.~Destefanis},
\authitem{L.~Fava},
\authitem{L.~Ferrero},
\authitem{M.~Greco},
\authitem{J.~Hu},
\authitem{L.~Lavezzi},
\authitem{M.~Maggiora},
\authitem{G.~Maniscalco},
\authitem{S.~Marcello},
\authitem{S.~Sosio},
\authitem{S.~Spataro}
\lastitem
\institem{Università di Trieste and INFN Sezione di Trieste,{ \bf Trieste}, Italy}
\authitem{R.~Birsa},
\authitem{F.~Bradamante},
\authitem{A.~Bressan},
\authitem{A.~Martin}
\lastitem
\institem{Uppsala Universitet, Institutionen för fysik och astronomi,{ \bf Uppsala}, Sweden}
\authitem{H.~Calen},
\authitem{W.~Ikegami Andersson},
\authitem{T.~Johansson},
\authitem{A.~Kupsc},
\authitem{P.~Marciniewski},
\authitem{M.~Papenbrock},
\authitem{J.~Pettersson},
\authitem{K.~Schönning},
\authitem{M.~Wolke}
\lastitem
\institem{The Svedberg Laboratory,{ \bf Uppsala}, Sweden}
\authitem{B.~Galnander}
\lastitem
\institem{Instituto de F\'{i}sica Corpuscular, Universidad de Valencia-CSIC,{ \bf Valencia}, Spain}
\authitem{J.~Diaz}
\lastitem
\institem{Sardar Patel University, Physics Department,{ \bf Vallabh Vidynagar}, India}
\authitem{V.~Pothodi Chackara}
\lastitem
\institem{National Centre for Nuclear Research,{ \bf Warsaw}, Poland}
\authitem{A.~Chlopik},
\authitem{G.~Kesik},
\authitem{D.~Melnychuk},
\authitem{B.~Slowinski},
\authitem{A.~Trzcinski},
\authitem{M.~Wojciechowski},
\authitem{S.~Wronka},
\authitem{B.~Zwieglinski}
\lastitem
\institem{Österreichische Akademie der Wissenschaften, Stefan Meyer Institut für Subatomare Physik,{ \bf Wien}, Austria}
\authitem{P.~Bühler},
\authitem{J.~Marton},
\authitem{D.~Steinschaden},
\authitem{K.~Suzuki},
\authitem{E.~Widmann},
\authitem{J.~Zmeskal}
\lastitem


==> components/sensors.tex <==
\section{Photon Sensors} \label{sec:sensors}

\subsection{Requirements}

The reconstruction of the Cherenkov image requires the reconstruction of two spatial coordinates. Additional measurements can be used to overconstrain the system and thus improve the detector performance and suppress background. Designs using two spatial coordinates plus a timing measurement in their reconstruction are known as 3D DIRC systems. The barrel DIRC for \panda 
relies mainly on the reconstruction of two spatial coordinates. A reasonably precise time information will be employed in aid of the reconstruction of the Cherenkov pattern and for background suppression.  

The envisaged detector system is subject to severe constructional constraints requiring the readout to be placed inside the solenoid of the \panda target spectrometer (TS). The expected field ranges up to 1.5 T. As magnetic shielding would decrease the geometrical coverage and thus hamper the performance of the detector, a highly efficient photon detection system insensitive to magnetic fields of that order of magnitude has to be identified and constructed.

Since the image planes will be rather compact and because the antiproton-proton average annihilation rate inside \panda will be $2\cdot10^7$, the single photon density at the sensor surface can reach 10 MHz/tube. This requires a very high rate stability and a long lifetime of the counters in terms of integrated anode charge. By measuring the time-of-propagation of the Cherenkov photons from their creation point to the sensor surface the $\pi$/K-separation can be optimized. However, to fully exploit this information a time resolution better than 100 ps ($\sigma$) is necessary. Finally, each particle traversing the radiators produces only few Cherenkov photons. As a consequence, the photon sensors have to be of very high quality in terms of quantum, collection and geometrical efficiency and require a low dark count rate.

The identification of the particle type relies on the reconstruction of the Cherenkov cone. This requires a position sensitive readout plane with a high ratio of active to passive surface. The best available options are improved multi-anode micro-channel plate PMTs. The current design of the Barrel DIRC foresees MCP-PMTs using a micro-channel plate of 10 $\mu$m pore diameter and a segmentation of $8\times 8$ pixels. 

\subsubsection{Magnetic field}
The compact design of the \panda target spectrometer requires the photon detection system 
and initial digitization stages to be located inside the return yoke of the target solenoid. The photon detection system of the Barrel DIRC is exposed to a magnetic field of about 1.0 T. The available construction space allows a moderate optimization of the PMT orientation relative to the magnetic field lines. The compact design and high geometrical filling factor necessary do not allow the installation of magnetic shielding. A suitable photon detection system should therefore work inside a magnetic field of up to 1.2 T (allowing for a safety margin of 20\% in the prediction of the magnetic flux).

%\begin{figure*}[htbp]
%\begin{center}
%\begin{minipage}{0.98\textwidth}
%	\includegraphics[width=1.0\textwidth,natwidth=610,natheight=642]{prototyping/pictures/albert/fig_magnet.png}
%\end{minipage}
%\end{center}
%\caption{ Magnetic field maps showing the strength of the solenoidal field in the EDD readout region}
%\label{fig:magnet}
%\end{figure*}


\subsubsection{Radiation Hardness}
The \panda experiment with hadronic interactions at high luminosity will produce
 a large integrated radiation dose that the detectors have to withstand. 
However, as \panda is a fixed target experiment most of the particles will be produced 
due to the Lorentz-boust into the forward direction. The photonsensors situated 
upstream with respect to the interaction point are less affected.
An integrated radiation dose corresponding to $10^{11}$ neutrons/cm$^2$ (which are the 
DATA for Barrel DIRC region???) is expected in this area over the lifetime of \panda, 
consisting mainly of neutrons and some electromagnetic background. This dose is not an issue for PMTs.



\subsubsection{Area and pixel size }

 The pixel size of the two-inch 8$\times$8 PHOTONIS Planacon MCP-PMTs or Hamamatsu H9500 MAPMTs is in the order of 6~mm. Since the liftime of the MCP-PMTs was significantly risen, it became possible to introduce a small EV into the solenoid.
To achieve the PID power required for \panda the photons are focused with a lens on the pixels in the focal plane on the back of the 30~cm deep EV which is equipped with 15~MCP-PMTs.
A further reduction of the pixel size will not enhance the performance much further without a significant redesign of the focusing optics.

\subsubsection{Time resolution}
The design of the Barrel DIRC requires time resolutions on the order of 100~ps. It is not 
suggested to use the photon time of propagation to reconstruct the Cherenkov angle or to 
mitigate dispersive effects. Time-resolution will however help in the event correlation and 
more important in the image reconstruction and background suppression. 

\subsubsection{Spectral range}
Cherenkov photons are produced in a "blue" spectrum as a function of the wavelength. The probability of emission decreases with the square of the wavelength, but the small wavelengths have the disadvantage of large dispersion effects.
The radiator material is transparent for visible and ultraviolet light and is not restricting the spectral sensitivity of candidate photon detection systems. The spectral range will be restricted to 
$\lambda > 300$ nm by the optical glue joints. 



\subsubsection{Rate}\label{subsubsection:rate}
The average interaction rates at \panda are estimated to be about 20~MHz at full luminosity. During short timescales  bursts of interactions can drive the rate up to 26 MHz. Each proton--antiproton interaction averages about two charged tracks that create Cherenkov light in the radiator of the Barrel DIRC. Each charged track in the radiator generates about a few hundred photons. About 20 of those that are focused and registered in the MCP-PMTs. Assuming that these are homogeneously distributed over all available channels one can derive the hit rates for the individual readout pixels as follows: 

pixel rate
\begin{eqnarray}
&=&\frac{2.6 \times 10^{7}  \frac{\text{events}}{\text{s}} \times 2  \frac{\text{tracks}}{\text{event}} \times 20  \frac{\text{photons}}{\text{track}}}{ 16  \text{ modules} \times 15\frac{\text{MCP-PMTs}}{\text{module}} \times 64\frac{\text{channels}}{\text{MCP-PMT}}}\\
&=&68\text{ kHz}
\end{eqnarray}
By adding a safety margin of a factor two because of possible charge sharing and cross-talk between pixels, a total count rate of about 136 kHz/channel  is achieved, keeping in mind that this value corresponds to extreme conditions where short burst temporarily create very high photon rates.


\subsubsection{Lifetime}
Simulations show that the expected photon rates at the readout plane of the Barrel DIRC will be in the MHz/cm$^{2}$ region for the highest luminosity. However, as far as lifetime calculations are concerned, it is important to average the interaction rates over the adequate lapse of time, namely one machine cycle of the HESR (compare chapter \ref{chap:panda}). Assuming a gain of 10$^{6}$ for the MCP-PMTs and 50\% duty cycle for \panda simulations predict that the integrated anode charge over 10 years can accumulate to about than 1 C/cm$^{2}$ for the Barrel DIRC. 

%%%\rot{Double check all numbers above!}


\subsection{Photon Devices}


\subsubsection{Microchannel-plate PMTs}

Micro-channel plate (MCP) photo multipliers are the ideal sensors for applications where a low noise and sub 100 ps single photon detection is required inside a high magnetic field. They are available as multi-anode devices and provide a good active area ratio while still being rather compact in size. However, until recently the major drawback of MCP-PMTs have been serious aging issues. Ions in the residual gas produced by the electron avalanche are accelerated towards the photo cathode (PC) which gets damaged from this permanent bombardment. As a consequence the quantum efficiency (QE) drops while the integrated anode charge increases. Until recently the rate conditions in \panda were far beyond the reach of any commercially available MCP-PMT where the QE had dropped by more than half after typically $<$200 mC/cm$^{2}$ \cite{nagoya, alex}, while for the Barrel DIRC 0.5 up to 2 C/cm$^{2}$ are needed to allow a detection of enough photons for the reconstruction of the Cherenkov angle. 

\begin{figure*}[htb]
\centering
%\includegraphics[width=.9\textwidth]{prototyping/hamamatsu.png}
\caption[Hamamatsu prototype]{The front and back sides of the Hamamatsu MCP-PMT prototype with 6x100 strips with a pitch of 0.5 mm}
\label{fig:hamamatsu1}
\end{figure*}

We have investigated the properties of many types of MCP-PMTs: circular-shaped single anode tubes of the Budker Institute of Nuclear Physics (BINP) in Novosibirsk, various quadratic-shaped 8$\times$8 pixel Planacon MCP-PMTs with different layouts of PHOTONIS, and several of the recently developed array R10754 with four strips or 16 pads of Hamamatsu.

Our comparative measurements of the lifetime of MCP-PMTs show clearly the enormous improvements of the most recent devices. The countermeasures against aging taken by the different manufacturers led to an increase of the lifetime by an order of magnitude and more. The most important observations are the fact that the ALD coated tubes show the best QE behavior. The $>$5 C/cm$^{2}$ integrated anode charge of the PHOTONIS XP85112 without a reduction of the QE make this device the most promising sensor candidate for the \panda DIRCs. New developments at Hamamatsu with a 2 inch-squared MCP-PMTs with ALD coating may also be an interesting option. Details of the lifetime issues are described in chapter \ref{ch:mcp_pmts}. 

\subsubsection{Multianode Dynode PMTs}

Multi-anode PMTs (MAPMTs) use a segmented anode and dynode structure to provide a correspondence between the position of the photon when entering the cathode and the readout pixel. The Hamamatsu H9500 series provides 256 3x3mm$^2$ pixels combined with a conventional 
photo cathode. The active area is 49x49mm$^2$ and the overall dimensions are very compact.  
The MAPMT provides an excellent packing density of 89\%. The outer dimensions make it a 
valid candidate for the Barrel DIRC photon detection system. The noise characteristics are very good as well. The PMT can be operated without preamplification. 
The quantum efficiency of the H9500 is given as 20\% at 420nm. The wavelength of maximum response is 420nm. The spectral response is 300 to 650 nm. 
This alone still allows to use this detector for the barrel DIRC. The main drawback lies in the sensitivity of these devices to magnetic fields. The gain drops rapidly even in small to moderate magnetic fields. The mechanical 
design and compactness prevents the installation of effective magnetic shielding. Additionally, 
the pixel-to-pixel uniformity of MAPMTs shows large deviations. The typical uniformity is 
quoted as 1:5. Last not least, the transit time spread of these MAPMTs is larger compared to 
MCP-PMTs hampering precise timing measurements.

%\clearpage



==> design/goalsandreqs.tex <==
\section{Goals and Requirements of the DIRC}
\label{cha:goalsandrequirements}

\subsection{Interferences with Neighbouring Detectors}
\label{sec:interferences}


==> panda/pandapid.tex <==
\section{The Particle Identification System} \label{sec:pandapid}
% \begin{figure*}[h]
% \begin{center}
% \includegraphics[width=.9\textwidth]{panda/stt-simu-dedx-seppower.png}
% \caption{
% Energy loss by a 40\% truncated mean algorithm for various particles 
% versus the reconstructed momentum (left) 
% and corresponding separation power (right) in the STT detector \cite{schepers2}.
% }
% \label{fig:stt-dedx-seppower}
% \end{center}
% \end{figure*}
The charged particle identification (PID) will combine time-of-flight,
tracking, dE/dx  and calorimetry information with the output from 
imaging Cherenkov detectors, with their focus on positive
identification of kaons.  

A RICH in the \panda Forward Spectrometer section is envisaged for smaller polar angles.


The individual \panda subsystems contributing to the PID
and the combination of their data into a global PID information
have been reviewed in the PID-TAG-report \cite{schepers2},
a subset of the findings is included below.





\subsubsection{Influence of the Radiation length to the EMC}

The presence of high material budget of other detectors in front of Electromagnetic Calorimeter (EMC) leads to the possibility for a high energetic photon to start a electromagnetic (EM) shower before the EMC called a pre-shower. 
Studies to the radiation length of the detector material in front of the EMC and its influence to the energy resolution of the EMC were done \cite{pre-shower}.
Figure~\ref{fig:mech-xmap} shows the accumulated radiation length~X$_0$. Clearly visible is, that the DIRC detector with its support structure and radiator material adds most to the possibility of a pre-shower. However, since the distance of the DIRC detector to the EMC is with less then 10cm very small. The resulting detoriation of the energy resolution of the EMC is plotted in Figure~{fig:EMC-presh-det}.


\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.9\columnwidth]{./design/pictures/EMC-xmap.jpg}
\end{center}
\caption{Map of the radiation length in front of the EMC.}
\label{fig:mech-xmap}
\end{figure}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.9\columnwidth]{./design/pictures/EMC-presh-det.jpg}
\end{center}
\caption{Detoriation of the energy resolution of the EMC due to pre-showers in the material on the way from the interaction point.}
\label{fig:EMC-presh-det}
\end{figure}

For a photon candidate of energy 1 GeV, the conversion probability inside the DIRC material is found to be 14\% at the polar angle of 90$^\circ$ increasing to 25\% at 22$^\circ$.

In \panda, a SciTil is situated in between the DIRC detector and the EMC. It has low material budget and is insensitive to $\gamma$, but it has a high efficiency to charged particles. In a study for BaBar experiment, it was shown that, by detecting pre-shower by DIRC itself, 50\% of the converted $\gamma$ can be recovered. But in our case, the separate SciTil detector would discover conversion with full efficiency and enhance the energy resolution.
We observed no distinct degradation of energy resolution due to the presence of DIRC pre-shower.
The EMC group provided beam test results where a 15~mm thick quartz bar was placed in front of the chrystals. The energy resolution at various energies of the incident photon with and without the quartz slab in front of the EMC material is shown in Figure~{fig:EMC-presh-beam-sim}.

\begin{figure}[!h]
\begin{center}
\begin{minipage}{0.49\textwidth}
	\includegraphics[width=0.93\textwidth]{./design/pictures/pre-shower-eres-beam.jpg}
	\newline
	\centering (a)
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
	\includegraphics[width=0.93\textwidth]{./design/pictures/pre-shower-eres-sim.jpg}
	\newline
	\centering (b)
\end{minipage}
\end{center}
\caption{EMC energy resolution over the $\gamma$ energy for beam tests (a) and for simulations (b)}
\label{fig:EMC-presh-beam-sim}
\end{figure}

There is no remarkable change in the energy resolution due to the presence of 15~mm thick quartz bar in front of EMC. This is also confirmed in pandaroot by changing the DIRC bar thickness to 15~mm.


\subsection{Muon Detection}

The return yoke for the solenoid magnet in the \panda TS
is laminated to accommodate layers of muon detectors.
As shown in Figure~\ref{fig:muon-layers} they form a range stack,
with the inner muon layer being able to detect low energy muons
and the cumulated iron layer thickness in front of the
outer layers providing enough hadronic material to stop
the high energy pions produced in \panda.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.95\columnwidth]{panda/tw20131203-13K_006_02.png}
\caption{
CAD drawing showing the muon detector layers sandwiched in between
the iron layers in the Barrel part of the return yoke.
}
\label{fig:muon-layers}
\end{center}
\end{figure}



% \subsection{Combined PID}

% The Particle Identification (PID) capability of several % candidate
% subsystem combinations (different tracker designs, TOF yes/no etc.)
% has been studied in the PID-TAG working group, and combined PID
% performances for all pairs from the set of (e, $\mu$, $\pi$, K, p)
% were presented in \cite{schepers2}.

% For the case of a STT tracker and no TOF subsystem the color
% Figure~\ref{fig:pid-tag_stt_notof} shows the $\sigma$ separation power
% for the $\pi$/K pairing as a function of polar angle and momentum.
% Positive identification of both particle types is required
% in order that a subsystem contributes a non-zero separation power.
% \begin{figure}[htb]
% \begin{center}
% \includegraphics[width=0.95\columnwidth]{panda/malgorzata-gumberidze-ipn-orsay_page15crop.png}
% %\includegraphics[width=70mm,trim = 83mm 76mm 91mm 64mm, clip]{panda/malgorzata-gumberidze-ipn-orsay_page15.pdf}
% %\includegraphics[scale=0.5,trim = 83mm 76mm 91mm 64mm, clip]{panda/malgorzata-gumberidze-ipn-orsay_page15.pdf}
% %\includegraphics{panda/out15page.pdf}
% \caption{Combined PID for K$^-$ without (left) and with DIRC detectors
% included on top of EMC and STT \cite{talk:pid:orsay}.
% The curves give kaon efficiencies,
% the red, green, blue and yellow lines
% refer to candidate lists with kaon purity selected to be
% Very Loose 20\%, Loose 30\%, Tight 55\% and Very Tight 70\%, respectively.
% }
% \label{fig:orsay-dsc}
% \vspace*{-4mm}
% \end{center}
% \end{figure}
% %figure from Orsay talk

% \begin{figure}[htb]
% \begin{center}
% \resizebox{.99\columnwidth}{!}{%
% \includegraphics[trim = 64mm 66mm 66mm 131mm, clip]{panda/pid-tag_stt_notof.pdf}}
% %\includegraphics{panda/out15page.pdf}
% \caption{
% Combined PID separation power for $\pi$-K pairing
% (from \cite{schepers2}). The color scale for the
% $\sigma$ separation power is given at the right edge of the figure. 
% This plot was generated including a previous version of the EDD.
% The current performance is described in chapter \ref{ch:performance}.
% }
% \label{fig:pid-tag_stt_notof}
% %\vspace*{-4mm}
% \end{center}
% \end{figure}
% %figure from PID-TAG


% %In this study of the PID-TAG group 
% %one looks into the combination of subsystems
% The EDD performance included in this PID-TAG study of 2008
% bases on a DIRC design status which has evolved since then.
% The performance values were obtained with a simulation \cite{foehl2009}
% of charged particles (non-decaying pions and kaons) with helix tracks
% in the approximation of a homogeneous magnetic field and material
% interaction through the radiator; Cherenkov photons generated,
% propagated through the optical system and recorded on position
% sensitive photon sensors. From these recorded hit patterns
% the charged particle velocity was then deduced.
% For the PID-TAG study the EDD performance has been computed
% for a raster of $\theta$ and momentum values within the subsystem
% phase space.

% It should also be noted that at far forward angles $\theta\leq 5^\circ$
% the optionally foreseen RICH of the Forward Spectrometer
% is included in this assessment.

% Simulations for physics channel studies
% which for the \panda experiment are now being performed in the
% FairRoot~/~PandaRoot framework require subsystem detector
% responses for individual particles. These are included
% into a PID analysis structure yielding PID probabilities 
% based on the Bayes method.
% Such Combined PID analysis in the PandaRoot framework
% has been studied \cite{talk:pid:orsay}. 
% For the performance of Barrel DIRC (DRC) and Disc DIRC (EDD; in the figure named DSC) a $\Theta_C$ versus $p$ parametrization is implemented in PandaRoot.
% The addition of DIRC data to the EMC and STT subsystems data
% in the analysis shows a clear jump in PID performance
% in the several GeV/c momentum range.






==> performance-validation/_region_.tex <==
\message{ !name(prototyping.tex)}
\message{ !name(prototyping.tex) !offset(449) }
\begin{table*}[htb]
\caption{Characteristics of the investigated lifetime-enhanced MCP-PMTs. Also shown is the currently accumulated anode charge of each measured MCP-PMT.}
\label{Tab:char}
{\small\begin{tabular*}{1.0\textwidth}[]{@{\extracolsep{\fill}}lllll}
\hline Manufacturer & BINP & PHOTONIS & Hamamatsu & Hamamatsu\\ 
\hline Type & & XP85112/A1-HGL & R10754X-01-M16 & R10754X-01-M16M \\
Counter ID & \#1359 / \#3548 & 9001223 / 9001332 & JT0117 & KT0001 / KT0002 \\
Pore diameter ($\mu$m) & 7 & 10 & 10 & 10 \\ 
Number of pixels & 1 & 8$\times$8 & 4$\times$4 & 4$\times$4 \\ 
Active area (mm$^{2}$) & 9$^{2}$ $\pi$ & 53$\times$53 & 22$\times$22 & 22$\times$22 \\ 
Total area (mm$^{2}$) & 15.5$^{2}$ $\pi$ & 59$\times$59 & 27.5$\times$27.5 & 27.5$\times$27.5 \\ 
Geometrical & & &  & \\ 
efficiency (\%) & 36 & 81 & 61 & 61  \\ 
\hline
% \multirow{2}{*}{Comments}
 & better vacuum; & better vacuum; & film between & ALD surfaces \\ 
Comments & new photo cathode & ALD surfaces & 1$^{st}$ \& 2$^{nd}$ MCP & \\ 
\hline
Integrated anode &  & &&\\
charge (mC/cm$^{2}$) & 3616 / 5025 & 5903 / 2375 & 2086 & 842 / 215     \\
\hline
\end{tabular*} 
}
\end{table*}
\message{ !name(prototyping.tex) !offset(-27) }


==> performance-validation/pid-performance.tex <==
Besides the pure technical performance of the detector design, the actual improvement in identifying different particle species by using the DIRC detector is of particular interest. In the PANDA context PID is quantified by specifying the separation power for two particles types. This quantity bases on the hypothesis of gaussian likelihoods for two species. It is defined as the difference between the center values of the Gaussian distributions expressed as the number of the average standard deviation
\begin{equation}
N_{\sigma} = \frac{|\mu_1-\mu_2|}{\sigma_1/2 + sigma_2/2}\quad .
\end{equation} 
The immediate advantage of this representation is, that it is independent from any kind of concrete combination of effciency, purity or level of mis-identification, being commonly used to quantify PID performance. It however is equivalent to a threshold on the likelihood, that results in the same fraction of efficiency loss and mis-identification level. The threshold itself has 

Within the PANDA software the PID information for charged particles is provided as the normalized product of the probability values computed from the likelihood functions of the individual PID-capable subdetectors. Even if the single likelihood has gaussian shape, the resulting probability distribution does not. Consequently the separation power cannot be computed directly according to the forumla above. 


==> sty/panda_commands.tex <==
% def_panda_cmd.tex
%
\RequirePackage[centertags]{amsmath}
%
\RequirePackage{xspace}
%\RequirePackage{ulem}
%
\def\MARK#1{\texorpdfstring{{\emph{\textcolor{red}{#1}}}}{{#1}}}
%\def\MARK#1{\emph{\textcolor{red}{#1}}}
%\def\MARK#1{{\bf \textcolor{red}{#1}}}
%\def\MARK#1{{#1}}
% use to mark text 
% (Text will be kept, but the marking removed in the final document)
%
\def\COM#1{\fbox{\parbox{\swidth}{\textcolor{red}{\bf COMMENT: #1}}}}
%\def\COM#1{}
% use to add comments
% (The whole will be removed in the final version)
%
% use to mark parts, which shouldn't be present in the cost-free version

\def\OnlyLayoutColumnBreak{{\vfill\newpage}}%

\def\OnlyLayoutPageBreak{{\vfill\clearpage}}%

\def\OnlyLayoutDoublePageBreak{{\vfill\cleardoublepage}}%

%
\def\bfg{\begin{figure}}%
\def\efg{\end{figure}}%
\def\bc{\begin{center}}%
\def\ec{\end{center}}%
\def\bi{\begin{itemize}}%
\def\ei{\end{itemize}}%
\def\be{\begin{equation}}%
\def\ee{\end{equation}}%
\def\bn{\begin{eqnarray}}%
\def\en{\end{eqnarray}}%
\def\ba#1{\left(\begin{array}{#1}}%
\def\ea{\end{array}\right)}%
\def\bef{\begin{equation}\fbox{$\displaystyle}%
\def\eef{$}\end{equation}}%
\def\bnf{\bef\ba{rcl}}%
\def\enf{\ea\eef}%
%\def\refeq#1{\Eqref{#1}\xspace}%
%\def\Refsec#1{sec.~\ref{#1}\xspace}%
%\def\Refchap#1{\Refchap{#1}\xspace}%
%\def\Reffig#1{\Reffig{#1}\xspace}%
%\def\Reftbl#1{\Reftbl{#1}\xspace}%
%\def\reftab#1{\Reftbl{#1}\xspace}%
\def\Refeq#1{Eq.~\ref{#1}\xspace}%
\def\Refeqs#1{Eqs.~\ref{#1}\xspace}%
\def\Refsec#1{Sec.~\ref{#1}\xspace}%
\def\Refchap#1{Chap.~\ref{#1}\xspace}%
\def\Reffig#1{Fig.~\ref{#1}\xspace}%
\def\Reffigs#1{Figs.~\ref{#1}\xspace}%
\def\Reftbl#1{Table~\ref{#1}\xspace}%
\def\Reftbls#1{Tables~\ref{#1}\xspace}%
\def\RefeqX#1{Eq.~\ref{#1}}%
\def\RefeqsX#1{Eqs.~\ref{#1}}%
\def\RefsecX#1{Sec.~\ref{#1}}%
\def\RefchapX#1{Chap.~\ref{#1}}%
\def\ReffigX#1{Fig.~\ref{#1}}%
\def\ReffigsX#1{Figs.~\ref{#1}}%
\def\ReftblX#1{Table~\ref{#1}}%
\def\ReftblsX#1{Tables~\ref{#1}}%
%\def\Reftab#1{Table~\ref{#1}\xspace}%
\def\ub{\underbrace}%
%
\def\vps{\hspace*{5mm}}%
\def\dsty{\displaystyle}%
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\lastitem{\ }%
\def\respitem#1{\institem{{\bf #1}\lastitem\\}}%
\let\groupitem=\authitem
%
\newcommand{\captionfonts}{\small}
%
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts {\bf #1:} #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts {\bf #1:} #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother   % Cancel the effect of \makeatletter
%
% a few commands to change the figure placing (commented are the default values)
%\renewcommand{\textfraction}{0.1} % 0.2
%\renewcommand{\bottomfraction}{0.4} % 0.3
%\renewcommand{\dbltopfraction}{0.8} % 0.7
%\renewcommand{\dblfloatpagefraction}{0.3} % 0.5
%\renewcommand{\floatpagefraction}{0.3} % 0.5
%\setcounter{dbltopnumber}{3} % 2
%\setcounter{bottomnumber}{2} % 1
%
\def\markpanda#1#2{\markboth{\Panda{} - #1}{FAIR/PANDA/#2}}%
%
% EOF: def_panda_cmd.tex


==> sty/panda_detector.tex <==
% panda_detector.tex
%
\RequirePackage{xspace}
%
\def\INST#1{\texorpdfstring{{\sf #1}}{{#1}}\xspace}%
%
\def\PANDA{\texorpdfstring{$\overline{\mbox{\sf P}}${\sf ANDA}}{Panda}\xspace}%
\def\Panda{\texorpdfstring{$\overline{\mbox{\sf P}}${\sf ANDA}}{Panda}\xspace}%
\def\panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\HESR{\INST{HESR}}%
\def\Hesr{\INST{HESR}}%
\def\GSI{\INST{GSI}}%
\def\Gsi{\INST{GSI}}%
\def\FAIR{\INST{FAIR}}%
\def\Fair{\INST{FAIR}}%
%
\def\Ts{TS\xspace}
\def\Fs{FS\xspace}
\def\Mvd{MVD\xspace}
%\def\Emc{EMC\xspace}
%\def\TsEmc{TS-EMC\xspace}
%\def\FsEmc{FS-EMC\xspace}
\def\Had{HAD\xspace}
\def\Muo{MUO\xspace}
\def\TsMuo{TS-MUO\xspace}
\def\FsMuo{FS-MUO\xspace}
\def\Stt{STT\xspace}
\def\Tpc{TPC\xspace}
\def\Dirc{DIRC\xspace}
\def\Rich{RICH\xspace}
\def\Mdc{MDC\xspace}
\def\TsMdc{TS-MDC\xspace}
\def\FsMdc{FS-MDC\xspace}
\def\Tof{TOF\xspace}
\def\Lum{LUM\xspace}
\def\Mag{MAG\xspace}
\def\TsMag{SOL\xspace}
\def\FsMag{DIP\xspace}
%
% EMC definitions
\def\Emc{EMC\xspace}
\def\BEMC{barrel EMC\xspace}
\def\FWEMC{forward endcap EMC\xspace}
\def\BWEMC{backward endcap EMC\xspace}
\def\TSEMC{target spectrometer EMC\xspace}
\def\FSEMC{forward spectrometer EMC\xspace}
\def\TsEmc{\TSEMC}
\def\FsEmc{\FSEMC}
%
\def\LAAPD{LAAPD\xspace}
\def\LAAPDs{LAAPDs\xspace}
\def\VPT{VPT\xspace}
\def\VPTs{VPTs\xspace}
\def\PWOII{PWO-II\xspace}
\def\PWO{PWO\xspace}
%
% EOF: def_panda_det.tex


==> sty/panda_symbols.tex <==
% def_panda_sym.tex
%
\input{./sty/pennames.sty}
\input{./sty/myunits.sty}
\input{./sty/mymath.sty}
%
\RequirePackage{xspace}
% Upright mu for micro
\DeclareFontFamily{U}{euc}{}% I chose euc because the chart is called Euler cursive
\DeclareFontShape{U}{euc}{m}{n}{<-6>eurm5<6-8>eurm7<8->eurm10}{}%
\DeclareSymbolFont{AMSc}{U}{euc}{m}{n} % I chose AMSc because AMSa and AMSb are defined in the amsfonts-package
\DeclareMathSymbol{\umu}{\mathord}{AMSc}{"16}
%
\def\degrees{\ensuremath{^\circ}\xspace}%
\def\percent{$\,$\%\xspace}%
\def\prm{\ensuremath{^\prime}}%
\def\etc{{\em etc.}\xspace}%
%
\def\tm{\texttrademark}
\def\tmr{\ensuremath{^{\textregistered}}}
%
\def\ppbar{\ensuremath{\mbox{p}\overline{\mbox{p}}}\xspace}%
\def\pbarp{\ensuremath{\overline{\mbox{p}}\mbox{p}}\xspace}%
\def\pbarA{\ensuremath{\overline{\mbox{p}}\mbox{A}}\xspace}%
\def\pbarN{\ensuremath{\overline{\mbox{p}}\mbox{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbar{\ensuremath{\overline{\mbox{p}}}\xspace}%
\def\nbar{\ensuremath{\overline{\mbox{n}}}\xspace}%
\def\pbarn{\ensuremath{\overline{\mbox{p}}\mbox{n}}\xspace}%
\def\nbarn{\ensuremath{\overline{\mbox{n}}\mbox{n}}\xspace}%
%
\def\qbar{\ensuremath{\overline{q}}\xspace}%
\def\cbar{\ensuremath{\overline{c}}\xspace}%
\def\ccbar{\ensuremath{c\overline{c}}\xspace}%
\def\ccbarg{\ensuremath{c\overline{c}g}\xspace}%
\def\cqbar{\ensuremath{c\overline{q}}\xspace}%
\def\cbarq{\ensuremath{\overline{c}q}\xspace}%
\def\uubar{\ensuremath{u\overline{u}}\xspace}%
\def\ddbar{\ensuremath{d\overline{d}}\xspace}%
\def\ssbar{\ensuremath{s\overline{s}}\xspace}%
\def\bbbar{\ensuremath{b\overline{b}}\xspace}%
\def\bqbar{\ensuremath{b\overline{q}}\xspace}%
\def\bbarq{\ensuremath{\overline{b}q}\xspace}%
\def\qqbar{\ensuremath{q\overline{q}}\xspace}%
\def\qqbarg{\ensuremath{q\overline{q}g}\xspace}%
\def\QQbar{\ensuremath{Q\overline{Q}}\xspace}%
%
\def\ee{\ensuremath{e^+e^-}\xspace}%
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}%
%
\def\piz{\ensuremath{\pi^0}\xspace}%
\def\pip{\ensuremath{\pi^+}\xspace}%
\def\pim{\ensuremath{\pi^-}\xspace}%
\def\pipm{\ensuremath{\pi^\pm}\xspace}%
\def\pimp{\ensuremath{\pi^\mp}\xspace}%
%
\def\K{\ensuremath{K}\xspace}%
\def\Kp{\ensuremath{K^+}\xspace}%
\def\Km{\ensuremath{K^-}\xspace}%
\def\Kpm{\ensuremath{K^\pm}\xspace}%
\def\Kmp{\ensuremath{K^\mp}\xspace}%
\def\KKbar{\ensuremath{K\overline{K}}\xspace}%
\def\Kz{\ensuremath{K^0}\xspace}%
\def\Kzbar{\ensuremath{\overline{K}^0}\xspace}%
\def\KzKzbar{\ensuremath{K^0\overline{K^0}}\xspace}%
\def\Ks{\ensuremath{K_S^0}\xspace}%
\def\Kl{\ensuremath{K_L^0}\xspace}%
%
\def\etaprime{\ensuremath{\eta\prm}\xspace}%
\def\pione{\ensuremath{\pi_1}\xspace}%
%
\def\uquark{\ensuremath{u}\xspace}%
\def\dquark{\ensuremath{d}\xspace}%
\def\squark{\ensuremath{s}\xspace}%
\def\cquark{\ensuremath{c}\xspace}%
\def\bquark{\ensuremath{b}\xspace}%
\def\tquark{\ensuremath{t}\xspace}%
%
\def\D{\ensuremath{D}\xspace}%
\def\Dbar{\ensuremath{\overline{D}}\xspace}%
\def\DDbar{\ensuremath{D\overline{D}}\xspace}%
\def\DpDm{\ensuremath{D^+D^-}\xspace}%
\def\Dz{\ensuremath{D^0}\xspace}%
\def\Dzbar{\ensuremath{\overline{D}^0}\xspace}%
\def\DzDzbar{\ensuremath{D^0\overline{D}^0}\xspace}%
\def\Dx{\ensuremath{D^\ast}\xspace}%
\def\Dxbar{\ensuremath{\overline{D}^\ast}\xspace}%
\def\DxDxbar{\ensuremath{D^\ast\overline{D}^\ast}\xspace}%
\def\Dxz{\ensuremath{D^{\ast 0}}\xspace}%
\def\Dxzbar{\ensuremath{\overline{D}^{\ast 0}}\xspace}%
\def\DbarDxx{\ensuremath{D\overline{D}^{\ast\ast}}\xspace}%
%
\def\Ds{\ensuremath{D_s}\xspace}%
\def\Dspm{\ensuremath{D_s^\pm}\xspace}%
\def\Dsmp{\ensuremath{D_s^\mp}\xspace}%
\def\Dsx{\ensuremath{D_s^\ast}\xspace}%
\def\Dsxpm{\ensuremath{D_s^{\ast\pm}}\xspace}%
\def\Dsxmp{\ensuremath{D_s^{\ast\mp}}\xspace}%
\def\DsDsbar{\ensuremath{D_s\overline{D_s}}\xspace}%
\def\DspDsm{\ensuremath{D_s^+D_s^-}\xspace}%
\def\DsxDsxbar{\ensuremath{D_s^\ast\overline{D_s}^\ast}\xspace}%
\def\DsbarDsxx{\ensuremath{\overline{D_s}D_s^{\ast\ast}}\xspace}%
%
\def\jpsi{\ensuremath{J\!/\!\psi}\xspace}%
\def\psiprime{\ensuremath{\psi\prm}\xspace}%
\def\etac{\ensuremath{\eta_c}\xspace}%
\def\etacprime{\ensuremath{\eta\prm_c}\xspace}%
\def\chicJ{\ensuremath{\chi_{cJ}}\xspace}%
\def\chiczero{\ensuremath{\chi_{c0}}\xspace}%
\def\chicone{\ensuremath{\chi_{c1}}\xspace}%
\def\chictwo{{\chi_{c2}}\xspace}%
\def\honec{\ensuremath{h_c}\xspace}%
%
\def\Cascade{\ensuremath{\Xi}\xspace}%
\def\Cascadebar{\ensuremath{\overline{\Xi}}\xspace}%
\def\LambdaLambdabar{\ensuremath{\Lambda\overline{\Lambda}}\xspace}%
\def\OmegaOmegabar{\ensuremath{\Omega\overline{\Omega}}\xspace}%
\def\SigmaSigmabar{\ensuremath{\Sigma\overline{\Sigma}}\xspace}%
\def\CascadeCascadebar{\ensuremath{\Xi\overline{\Xi}}\xspace}%
%
\def\kev{{\mbox{keV}}\xspace}%
\def\kevcc{{\mbox{keV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mev{{\mbox{MeV}}\xspace}%
\def\mevc{{\mbox{MeV}\!/\!\mbox{\em c}}\xspace}%
\def\mevcc{{\mbox{MeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mevccsq{{\mbox{MeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\gev{{\mbox{GeV}}\xspace}%
\def\gevc{{\mbox{GeV}\!/\!\mbox{\em c}}\xspace}%
\def\gevcsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevcc{{\mbox{GeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevccsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
%
\def\aC{{\mbox{aC}}\xspace}%
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\mubarn{\ensuremath{\rm \,\mu b}\xspace}
\def\nb{\ensuremath{\rm \,nb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
%
\def\JPC{\ensuremath{J^{\!P\!C}}\xspace}%
\def\JPCzeropm{\ensuremath{0^{+-}}\xspace}%
\def\JPCzeropp{\ensuremath{0^{++}}\xspace}%
\def\JPCzeromm{\ensuremath{0^{--}}\xspace}%
\def\JPCzeromp{\ensuremath{0^{-+}}\xspace}%
\def\JPConepm{\ensuremath{1^{+-}}\xspace}%
\def\JPConepp{\ensuremath{1^{++}}\xspace}%
\def\JPConemm{\ensuremath{1^{--}}\xspace}%
\def\JPConemp{\ensuremath{1^{-+}}\xspace}%
\def\JPCtwopm{\ensuremath{2^{+-}}\xspace}%
\def\JPCtwopp{\ensuremath{2^{++}}\xspace}%
\def\JPCtwomm{\ensuremath{2^{--}}\xspace}%
\def\JPCtwomp{\ensuremath{2^{-+}}\xspace}%
%
\def\JPCscalar{\JPCzeropp}%
\def\JPCvector{\JPConemm}%
\def\JPCtensor{\JPCtwopp}%
%
\def\extl{\ensuremath{E_{xtl}}\xspace}
\def\ecl{\ensuremath{E_{cl}}\xspace}
\def\emax{\ensuremath{E_{max}}\xspace}
% EOF: def_panda_sym.tex

